Turning Flowchart into Dialog: Augmenting Flowchart-grounded Troubleshooting Dialogs via Synthetic Data Generation

Flowchart-grounded troubleshooting dialogue (FTD) systems, which follow the instructions of a flowchart to diagnose users' problems in specific domains (e.g., vehicle, laptop), have been gaining research interest in recent years. However, collecting sufficient dialogues that are naturally grounded on flowcharts is costly, thus FTD systems are impeded by scarce training data. To mitigate the data sparsity issue, we propose a plan-based synthetic data generation (PlanSDG) approach that generates diverse synthetic dialog data at scale by transforming concise flowchart into dialogues. Specifically, its generative model employs a variational-base framework with a hierarchical planning strategy that includes global and local latent planning variables. Experiments on the FloDial dataset show that synthetic dialogue produced by PlanSDG improves the performance of downstream tasks, including flowchart path retrieval and response generation, in particular on the Out-of-Flowchart settings. In addition, further analysis demonstrate the quality of synthetic data generated by PlanSDG in paths that are covered by current sample dialogues and paths that are not covered.

==> experiment.tex <==
\section{Experiments}

\setlength{\tabcolsep}{4pt}
\begin{table*}[t]
\small
\centering
%\resizebox{0.99\textwidth}{21mm}
{
\begin{tabular}{l|ccccccc}
\toprule[1pt]
   Model  & PPL & BU-4 & RG-L  &  Dist-2 & Emb (Avg/Extr/Gre) & BERTScore (P/R/F1) & BARTScore  \\
  \hline
  GPT-2 (large) & 24.051 & 0.268 & 0.431 & 0.267  &  0.881/0.687/0.841 & 0.869/0.851/0.859 & -2.590 \\
  BART (large) & 33.914 & \textbf{0.297} & 0.472  & 0.351 & 0.872/0.675/0.833 & 0.884/0.877/0.880 & -2.164 \\
  DialoGPT (large) & 27.785 & 0.247 & 0.401  & 0.366 & \textbf{0.893}/0.625/0.826 & 0.864/0.848/0.856 & -2.328 \\
  BlenderBot & \textbf{21.936} & 0.193 & 0.356  & 0.308 & 0.826/0.593/0.786 & 0.836/0.851/0.844 & -2.051 \\
  \hline
  Our model & 31.266 & 0.285 & \textbf{0.512}$^\star$  & \textbf{0.397}$^\star$ &  0.861/\textbf{0.694}/\textbf{0.857}$^\star$ & 0.872/0.864/0.867 &  \textbf{-2.037}  \\
  
 \bottomrule[1pt]
\end{tabular}}
\vspace{-2mm}
\caption{Intrinsic evaluation results for pseudo dialogue generation. The metrics  Perplexity, BLEU-4, ROUGE-L, Distinct-2 and Embedding are
abbreviated as PPL, BU-4, RG-L, Dist-2 and Emb respectively. The best results are highlighted with \textbf{bold}. ``$^\star$'' denotes that a result is statistically significant with $p < 0.01$. \reza{remove bertscore}}
\label{tab_auto-eval}
\end{table*}


\subsection{Experimental Setup}
\label{section:expsetup}

\textbf{Dataset.} The \textit{FloDial} dataset is collected for the troubleshooting situations, where the interactions between user and agent are carried to diagnose user's problem in specific domain. \textit{FloDial} contains two main domain: vehicle and laptop. Each domain contains 5 sub-problems. For each sub-problem, there is a corresponding flowchart. Dialogues are conducted based on these flowcharts.  Details about each sub-problems and flowchart are shown in Table~\ref{tab:flodial}. \textit{FloDial} contains 1,789 dialogue sessions in total. In the experiments of \textit{FloDial} paper, they construct two settings: in-domain and out-domain settings. The test set of in-domain setting contains the dialogue in 8 sub-problems (including ticking, brake, battery, wont\_start, drive, overheating, power and lcd), which maintains the same domain with training set. Beside, the test set of out-domain setting only contains 2 sub-problems (engine, wireless), while all other 8 sub-problems are treated as training set. An example of flowchart in \textit{car\_wont\_start} domain is shwon in Figure~\ref{ex:flow}

\begin{table}[t]
    \centering
    \scriptsize
    \begin{tabular}{c|ccccc}
    \toprule
       Domain  & \multicolumn{5}{c}{Vehicle}  \\\hline
        ~ & ticking & brake & battery & wont\_start & engine \\\hline
        \#Dialog & 178 & 188 & 196 & 174 & 168 \\\hline
        \#sub-path & 15 & 19 & 18 & 17 & 14 \\\hline\hline
        Domain  & \multicolumn{5}{c}{Laptop}  \\\hline
        ~ & drive & overheating & power & lcd & wireless \\\hline
        \#Dialog & 192 & 186 & 188 & 178 & 196 \\\hline
        \#sub-path & 16 & 13 & 15 & 15 & 15 \\\hline\hline
        
    \end{tabular}
    \caption{\#Dialog and \#sub-path denote the number of dialogue session, and the number of sub-paths of each corresponding flowchart.}
    \label{tab:flodial}
\end{table}


\begin{figure}
    \centering
    \small
    \includegraphics{images/car_wont_start.JPG}
    \caption{The flowchart example of \textit{car\_wont\_start} domain. The figure is directly downloaded from the website:\url{https://www.ifitjams.com/}, the original source of \textit{FloDial} dataset.}
    \label{ex:flow}
\end{figure}


Besides, as the original \textit{FloDial} dataset does not contain any dialogue act information, we manually label the dialogue act for each dialogue utterance. The selection of dialogue acts is based on the investigation on previous work, including Switchboard (\url{https://catalog.ldc.upenn.edu/LDC97S62}), AMI (\url{https://groups.inf.ed.ac.uk/ami/corpus/}), MultiWoz~\cite{budzianowski2018multiwoz} and etc. The statistical results on the high-frequency dialogue act is shown in Figure~\ref{ex:da}. Finally, we chose seven most frequent dialogue, which also compatible with the \textit{FloDial} dataset. These dialogue acts include: \{statement, inform, yes-no-question, clarification, thanking, closing and suggestion\}. The percentage of each dialogue act in the \textit{FloDial} is: statement: 11.6\%, inform: 34.7\%, yes-no-question: 26.2\%, clarification: 9.8\%, thanking: 6.2\%, closing: 4.3\% and suggestion: 7.2\%.
% \textbf{Dataset.} We use the \textit{FloDial} dataset~\cite{flowchart2021emnlp} for our experiments. \textit{FloDial} is a troubleshooting dialogue dataset containing ten flowcharts and 1,798 dialogues in total. It has two main domains: vehicle and laptop --- each domain deals with five sub-problems. On average, there are 17.8 sub-paths in one flowchart. There are two different test settings in \textit{FloDial}: In-domain and Out-domain. In the In-domain setting, the training and test sets share the same flowcharts, while in the Out-domain setting, the training set contains eight flowcharts, and the test set contains the remaining two flowcharts. We keep the same test set as in the original paper for our evaluation.

\noindent \textbf{Baselines.} We select four strong pre-trained models as our baselines, containing two language models and two conversational models. These four baselines are: GPT-2, BART, DialoGPT and BlenderBot. In our experiment, we employ the fine-tuning strategy for the baselines and our model, as it outperforms prompt-tuning for generating valid dialogue data. The implementation details and reproduction checklist can be found in the Appendix.

\noindent\textbf{Evaluation metrics.} We perform intrinsic and extrinsic evaluation.

Our intrinsic evaluation assesses the fluency, diversity and semantic coherence (with the flowchart) of the synthetic dialogues. Fluency is assessed using Perplexity (PPL), BLEU~\cite{papineni2002bleu} and ROUGE~\cite{lin2004rouge}; diversity is assessed with Distinct~\cite{li2016distinct}; and semantic coherence is evaluated using %%BERT-Score~\cite{zhang2019bertscore},
Embedding Metrics (Average, Extrema, Greedy) and BART-Score~\cite{yuan2021bartscore}.

Our extrinsic evaluation determines whether augmentation with our synthetic data improves the performance of state-of-the-art \FTDs\ in terms of response generation and information retrieval from the flowchart.

% metrics: (1) Fluency and Naturalness: Perplexity (PPL), BLEU, ROUGE.
%          (2) Diversity: Distinct\footnote{\url{https://github.com/Maluuba/nlg-eval}}
%          (3) Semantic Coherence: BERTScore\footnote{\url{https://github.com/huggingface/evaluate}}, Embedding Metrics (Average, Extrema, Greedy)
%          (4) Content Fidelity:  RoBERTa-NLI~\cite{dusek2020evaluating} evaluation metric\footnote{\url{https://github.com/ufal/nlgi_eval}}.
%          PARENT~\cite{dhingra2019handling}

\subsection{Intrinsic Evaluation}
As seen in Table~\ref{tab_auto-eval}, VarDA outperforms the baselines in terms of RG-L, Dist-2, Embedding and BART-Score. For PPL, BLEU-4 and BERT-Score, the results of VarDA are close to the baseline models. The significant improvement obtained by VarDA for Dist-2 indicates that our model is able to generate more diverse content than the baselines --- a result of our latent variable modeling. The high scores of Embedding BART-Score indicate that our model also has the capability to generating utterances that are semantically coherent with the input flowchart. 

\begin{comment}
%%IZ: this is not relevant
In addition, we observed that general pre-trained models (\eg\ GPT-2, BART) maintain better performance than conversational pre-trained models (\eg\ BlenderBot, DialoGPT) in terms of coherence and language fluency. This interesting phenomenon might be due to the fact that general pre-trained models  are learned from massive training corpora, which facilitates better generalization to various conversation topics.
\end{comment}

\subsection{Extrinsic Evaluation}
Here we use Perplexity and BLEU to evaluate response generation performance, and Recall@1 and Recall@5 to assess information retrieval performance.
As seen in Table~\ref{tab:aug}, XXX

\begin{table}[!t]
    \centering
    \small
    \begin{tabular}{l|cccc} \hline
      Data Size   & \multicolumn{4}{|c}{Seen In-domain}  \\ \hline
       ~ & PPL & BLEU & R@1 & R@5  \\ \hline
       %reproduced-1 (1x) & 4.63 & 20.58 & 0.828 & 0.951  \\ \hline 
       FloNet (1x) & 4.93 & 19.36 & 0.834 & 0.957   \\ \hline 
       2x data & 5.26 & 20.72 & 0.843 & 0.956 \\ \hline
       5x data & 4.28 & 21.06 & 0.851 & 0.961 \\ \hline
       10x data & 4.35 & 21.18 & 0.853 & 0.968\\ \hline\hline
       Data Size &  \multicolumn{4}{|c}{Unseen Out-domain} \\ \hline
        ~ & PPL & BLEU & R@1 & R@5  \\ \hline
       %reproduced-1 (1x) & 10.491 & 10.824 & 0.543 & 0.782 \\ \hline
       FloNet (1x) & 17.084 & 9.533 & 0.529 & 0.765 \\ \hline
       2x data & 13.274 & 11.751 & 0.546 & 0.819 \\ \hline
       5x data & 15.628 & 14.002 & 0.595 & 0.837 \\ \hline
       10x data & 12.638 & 14.725 & 0.609 & 0.841 \\ \hline
    \end{tabular}
    \caption{Extrinsic performance. Results of reproduced 1 are from their provided checkpoint. Results of reproduced 2 are from training from scratch.}
    \label{tab:aug}
\end{table}

% \subsection{Experiment 2}

% In different data size, whether these model can help improve the performance of original flowchart dialogue systems, in terms of response generation and flowchart node retrieval.


% \subsubsection{Experiment 3}

% Comparison and analysis on the distribution discrepancy between original dataset and pseudo synthetic dataset. 


% \subsubsection{Experiment 4}
% Case studies on the pseudo dialogue generation. Show some cases.

% \subsubsection{Experiment 5}
% Hallucination phenomenon analysis of pseudo dialogue generation.

==> introduction.tex <==
\section{Introduction}
%%FTDs are important
%%However, there are no datasets for FTDs (The closest to date is troubleshooting systems (without flowcharts) Wei et al 2018).
%%The first attempt at developing a dataset for FTDs is Flodial. However, despite the large development effort, this dataset doesn't cover the whole flowchart (and it has other problems -- it is very rigid -- maybe mention in lit survey, or in limitations section).
%%Data augmentation has been used in the past to supplement datasets in [list areas]. However, the methods proposed to date are not suitable for FTDs (explain in Section 2).
%%In this paper, we propose a data augmentation method for ... . Our method comprises ... 

%% FTDs are important
%% The tasks for TSDs are understanding a problem description, determining the root cause of the problem, and providing a solution. 
%% Why are we talking about recommender systems?
{\em Flowchart-grounded Troubleshooting Dialogue Systems} ({\em \FTDs}\/)~\cite{leake2005using,boye2007dialogue,wei2018task,flowchart2021emnlp} communicate with users to help them diagnose problems in vertical domains (\eg\ vehicle, laptop) --- the dialogue agent must identify a problem by asking users a series of questions according to the instructions in a flowchart. 
%
{In contrast with typical task-oriented dialogue systems where the main task is to satisfy user requests by recommending an appropriate target~\cite{wen2017network,budzianowski2018multiwoz}, troubleshooting dialogues must perform various tasks, including understanding a problem description, determining the root cause of the problem precisely, and providing a solution. }%\noteIZ{I don't see a fundamental difference: when satisfying requests, we must understand the problem} 
%
As shown in Figure~\ref{fig:intro}, a dialogue agent follows a path in a flowchart to resolve users' problems. Thus, previous work for typical recommender dialogue systems cannot be applied to model \FTDs\  directly.
%%\FTDs\ have the potential of being useful in many scenarios. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.99\linewidth]{images/flow_intro.pdf}
    \caption{A sample flowchart-grounded troubleshooting dialogue.}
    \label{fig:intro}
\end{figure}

%% To date, the closest to FTDs is troubleshooting systems. For example ... . But there is no work on FTDs because of the dearth of datasets. In fact, the first dataset developed for FTDs is ...

Several methods have been developed to model troubleshooting dialogues~\cite{boye2007dialogue,williams2007applying,williams2007using,paek2008automating,janarthanam2008user,wei2018task}. 
%
%\rezaTrack{Ingrid: It wold be good to cite a few pioneering papers for troubleshooting from early days; your suggestions are appreciated.}
%
For example, \citet{boye2007dialogue} proposed a hand-coded method for the scenario of Internet connections. 
\citet{williams2007applying} upgraded preamble method by applying  Markov decision processes (MDP) to precisely track user's goal and action.
\citet{wei2018task} built an end-to-end system for disease diagnosis in a healthcare scenario. 
%
%However, we could not find \FTD\ corpora in open resources, which hinders development in this field. Therefore, crowd-sourcing flowchart-grounded dialogues from human is an alternative method.
%
%%\trackHZ{\citet{flowchart2021emnlp} crowd-sourced a dataset {\em FloDial} containing ten flowcharts (Section~\ref{section:expsetup}), and about 180 dialogues for each flowchart. Even though extensive human labor have been taken for this corpus, the dialogues in it cover only 60\% of the paths in flowcharts on average (Figure~\ref{fig:stat}). Overall, crowd-sourcing sufficient large corpora that can cover all the situations in flowcharts is challenging and time consuming. }
%
But there is no work on FTDs because of the dearth of datasets. In fact, the first dataset developed for FTDs is {\em FloDial}~\cite{flowchart2021emnlp} through crowd-sourcing, containing  1,789 dialogues about ten flowcharts (Section~\ref{section:expsetup}).
%\citet{flowchart2021emnlp} crowd-sourced a dataset {\em FloDial} of 1,789 dialogues about ten flowcharts (Section~\ref{section:expsetup}). 
%Even though this is a relatively large corpus, 
Even though it already has taken great human effort, the dialogues in \textit{FloDial} still cover only 65\% of the paths in flowcharts on average (Figure~\ref{fig:stat}). 
Therfore, collecting a sufficiently large flowchart-related dialogue corpus for \FTDs\ is challenging, particularly as it requires domain experts and professional knowledge of flowcharts.

%Overall, crowd-sourcing sufficient large corpora that can cover all the situations in flowcharts is challenging and time consuming. 
%%\trackIZ{\bf You are contradicting yourself. In one paragraph, you say that flowcharts require domain knowledge, and then you say the corpus can be crowdsourced, which one is it? Also, plz fix Figure 2 as I requested}

%%%%%%%%%% This paragraph will be commented out %%%%%%%%%%%%%%%%%%%
\begin{comment}
However, it is commonly observed that \FTDs\ usually require \trackIZ{professional and specific knowledge of flowcharts.}\noteIZ{Of the domain or the flowchart?} \noteHZ{flowchart is the representative of domain knowledge, so for here I suppose that flowchart = domain. Agree or Disagree?} \trackIZ{Therefore, collecting a sufficiently large corpus of flowchart-related dialogues is usually time consuming and labor intensive.}\noteIZ{I don't see how this conclusion follows} \citet{flowchart2021emnlp} crowd-sourced a dataset of 1,789 dialogues about ten flowcharts (Section~\ref{section:expsetup}). However, as shown in Figure~\ref{fig:stat}, the dialogues in this corpus cover only 60\% of the paths in the flowcharts on average.\noteIZ{Make the picture only about covered paths}
\end{comment}
%%%%%%%%%% This paragraph will be commented out %%%%%%%%%%%%%%%%%%%
Data augmentation can be an effective approach for extending a training corpus. However, previous data augmentation methods in dialogue research mainly focused on two areas:
NLU in slot-filling task-oriented dialogues and response generation in open-domain dialogues. Data augmentation for NLU  typically synthesizes single labels (\eg\ intent, dialogue act) rather than utterances or complete dialogues. Data augmentation for  response generation  synthesizes pseudo utterances, which are generally based on retrieval from external resources~\cite{cai2020data,kann2022open}. However, such resources are unavailable for \FTDs. %\noteRH{can we also mention "not suitable" and then mention why?}
%\trackIZ{What was done in NLU, and why it isn't suitable} \eg\ intent detection, dialogue act classification~\cite{wen2016network}.
%Data augmentation for response generation in open-domain dialogues are retrieval-based, using phrases obtained from external resources~\cite{cai2020data,kann2022open}. To the best of our knowledge, such resources are not available for \FTDs.
%%Therefore, few work shed light on synthesizing complete dialogues for FTDSs.

% there is relatively little research on them due to the limited access to large-scale datasets. Unlike typical open-domain~\cite{ma2021unstructured} or traditional slot-filling task-oriented dialogue systems~\cite{wen2016network} which have already got sufficient dataset, it is quite labour intensive and time consuming to collect a large-scale corpus for such complex troubleshooting scenarios at this stage. \citet{flowchart2021emnlp} collected a dataset of 1,789 dialogues about ten flowcharts for this task (Section~\ref{section:expsetup}). However, as shown in Figure~\ref{fig:stat}, these dialogues do not cover all the situations in the flowcharts.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/stat_new.pdf}
    \caption{Statistics on the percentage (\%) of (un)covered paths in the \textit{FloDial} (containing ten flowcharts in Vehicle and Laptop  domains respectively)-- each flowchart pertains to a specific vehicle problem. In total, more than 35\% of paths are not covered by dialogue instances.}
    \label{fig:stat}
    \vspace*{-3mm}
\end{figure}

%%\trackHZ{As there is no appropriate augmentation approach for \FTDs\ at this stage,}\
In this paper, we explore data augmentation approach with pre-trained models that  automatically synthesizes complete pseudo dialogues for \FTDs. Our approach enjoys the following desiderata. Firstly, it models discourse relations between utterances to realise  dialogue acts (\eg\ inform, clarify). Secondly, it controls the diversity of expressions. Thirdly, it ensures content faithfulness of the synthetic dialogue to the underlying flowchart.
%\noteIZ{why haven't these tasks been tackled in slot-filling dialogues?}\\
%\trackHZ{For NLU tasks in slot-filling dialogues, it's not difficult. But we formulate our augmentation method as a generation task. This is difficult, and not explored in previous dialogue research.} 
%\trackIZ{\bf You are not explaining why it is not difficult in SLU, and you are confusing SLU with slot filling dialogues, which one is it?} 
%\trackHZ{previous augmentation on NLU is to synthesize single labels (e.g., intent, slot, dialogue act) giving an unlabelled dialogue context, rather than generating a complete dialogue.}
We further investigate the performance of generic pre-trained models (\eg\ GPT-2, DialoGPT) for synthetic dialogue generation. Despite the ability of these models in generating fluent and natural-looking utterances, we find that they usually fall short in incorporating appropriate dialogue specific features, \eg\ dialogue acts and flowchart information.
%\textcolor{red}{****the following sentence will be commented out.}  and find \trackIZ{it not easy}\noteIZ{Huh?}\noteHZ{Rephrase} to synthesize diverse and coherent dialogue content. These models are able to generate fluent and natural sentences, but fall short on generating \trackIZ{dialogue-specific features}.\noteIZ{Huh?} \textcolor{red}{****the above sentence will be commented out.} 

{To this end,} we propose a {\em Variational Data Augmentation} ({\em VarDA}\/) approach for generating pseudo dialogues for \FTDs. VarDA takes as input a path in the underlying flowchart (Figure~\ref{fig:intro}), and generates a dialogue session consisting of dialogue acts, content, and utterances. It
employs a hierarchical planning strategy which includes \textit{global} and \textit{local} latent planning variables. %\rezaTrack
{The \textit{global} latent variable is responsible for modeling the dialogue acts between the the dialogue turns, providing a high-level sketch. 
%
%The \textit{local} latent variables control the diversity of synthetically generated utterances
To be able to model these global variables, we manually label the dialogue acts for the utterances in the \textit{FloDial} dataset.
For sentence realization, we utilize the \textit{local} latent variable to control the diversity of these synthetic dialogues. }

% To tackle these problems, we firstly investigate the use of pre-trained models, and find it not easy to synthesize diverse and coherent dialogue content. Then, we propose a Variational-based Data Augmentation (VarDA) method for \FTDs. This method is able to automatically synthesize new pseudo dialogue instances, as well as maintain high quality and diversity. To better model the complex structure of flowchart-based troubleshooting dialogues, we propose a planning-based hierarchical variational model. Generally, each turn in a dialogue conveys a communicative goal known as dialogue act, which structures the dialogue in further~\cite{thorne2017chatbots}. Therefore, we firstly utilize dialogue act information as the high-level structure planning, and propose to learn a latent variable sequence with each latent code as the sketch for further local dialogue context realization. Then, we employ the low-level latent  variable to  generate each of the individual dialogue context conditioned on the sequence of dialogue act.

% To fulfil the requirements of expressions diversity, this model is capable to inject variations at both high-level planning and low-level realization with the hierarchical latent structure. At high-level sketch, we introduce a global planning latent variable to model the diversity of dialogue acts. At low-level sentence realization, we introduce a local latent variable for dialogue utterance generation.


We conduct our experiments based on \textit{FloDial} dataset from both \textit{intrinsic} and \textit{extrinsic} evaluation.
Results on \textit{intrinsic} evaluation demonstrate that synthetic dialogue content produced by VarDA outperform strong baseline models in term of diversity and faithfulness. In addition, \textit{extrinsic} evaluation is conducted to study the augmentation performance on downstream tasks: flowchart path retrieval and response generation. Synthetic data produced by VarDA has better augmentation effects, compared to those data synthesized by strong baseline models. Moreover, we observe that our VarDA model can generate acceptable pseudo dialogues for unseen flowcharts, which has the potential to improve the performance of FTDSs in uncovered scenarios.


%Our experimental results show that our proposed VarDA model outperforms several baselines in terms of diversity and faithfulness to the flowchart. In addition, we experiment with different size corpora of synthesized dialogue data to augment troubleshooting dialogues. Our results show that the synthetic dialogues produced by VarDA improve the performance of state-of-the-art \FTDs\ in both in-domain and out-of-domain settings, in terms of flowchart path retrieval and response generation.

% We summarize our contributions in three folds:

% (1) We propose a novel data augmentation method for flowchart-based troubleshooting dialogue systems.

% (2) We devise a planning-based hierarchical variational model to support our data augmentation process, considering a high-level structure planning by utilizing dialogue act information, and a low-level utterance realization based on the flowchart and external knowledge base.

% (3) From the experimental perspectives ......

% outline:

% \textbf{Paragraph 1:} (1) Introduction about the basic function and application scenarios of troubleshooting dialogue systems. (2) Differences between trouble-shooting dialogue systems and traditional slot-filling based task-oriented dialogue systems.

% \textbf{Paragraph 2:} (1) Illustrate the data scarcity problem in the troubleshooting dialogue systems. and why it hampers the performance.
% (2) Main problem: impeding the performance of existing systems. (3) sub-problem 1: the limited data size impedes the performance of existing systems. (Use a figure to illustrate, e.g. performance discrepancy with 1x, 2x, 5x, 10x data size) (4) sub-problem 2: limited data cannot cover all situations in specific domains, e.g. in flowchart dataset, not all flowchart paths are covered by dialogue content (Use a figure to illustrate the rate of uncovered ).


% \textbf{Paragraph 3:} (1) we investigate the use of pre-trained models, and find it not easy to synthesize diverse and coherent dialogue content, Then, present an variational generative model to generate diverse and coherent pseudo dialogue. The remaining part will introduce the details of our proposed variational generative model.

% \textbf{Paragraph 4:} Experiment results and new findings.

% \textbf{Paragraph 5:} Summarization of our contributions.


% \begin{table}[t]
%     \centering
%     \small
%     \begin{tabular}{c|ccccc} \hline
%       Type   & \multicolumn{5}{|c}{Car} \\ \hline
%       ~ & lcd &  brake & battery & engine & wont\_start\\ \hline
%       total & 15 & 19 & 18 & 14 & 17\\ \hline
%       covered & 10 & 11 & 10 & 9 & 9 \\ \hline
%       uncovered & 5 & 8 & 8 & 5 & 8 \\ \hline
%       ~   & \multicolumn{5}{|c}{Laptop} \\ \hline
%       ~ & drive &  over\_heat & power & ticking & wireless \\ \hline
%       total & - & - & - & - & - \\ \hline
%       covered & - & - & - & - & - \\ \hline
%       uncovered & - & - & - & - & - \\ \hline

%     \end{tabular}
%     \caption{paths statistics that covered and uncovered.  }
%     \label{tab:aug}
% \end{table}

==> introduction_haolan_v2.tex <==
\section{Introduction}
\textcolor{blue}{Task-oriented dialogue systems (TODs) are designed to complete specific tasks through conversation with human, e.g.,  ticket booking~\cite{wen2016network} or problem diagnosis~\cite{boye2007dialogue,flowchart2021emnlp}. To achieve their goals, TODs usually require relevant and specific domain knowledge from external databases or online APIs. 
%To build competitive TOD systems, it is necessary to collect sufficiently large dialogue instances as training data.
While independent  knowledge bases or dialogue corpora are abundant on the website, it is costly and laborious to align them well as underlying domain-specific training data.
Directly crowd-sourcing dialogues can also be challenging: crowd-workers are rarely domains experts with massive task-specific knowledge and tend to provide shallow dialogue content~\citep{li-etal-2022-ditch}. Therefore,  it is difficult to collect enough training data for a specific domain in a short period time. }


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.99\linewidth]{images/flow_intro_acl2023.pdf}
    \caption{A sample flowchart-grounded troubleshooting dialogue. Agent follows the path of a flowchart to help user diagnose  problems.}
    \label{fig:intro}
\end{figure}


\textcolor{blue}{To overcome this challenge, some recent work utilize data augmentation algorithm to generate synthetic data. However, existing data augmentation approaches, \eg\ back-translation~\citep{zhang-zong-2016-exploiting}, EDA~\citep{wei-zou-2019-eda} and PARG~\cite{gao2020paraphrase} , only replace the surface tokens or paraphrase sentences, and retain their semantic meaning. As a result, these methods are limited to produce new synthetic data conditioned on previously covered knowledge.
%they are limited to produce diverse synthetic data in semantic.
Observing that high-quality knowledge base, \eg\ structured flowchart and database, are abundant, it would yield enormous corpora for low-resource TODs if we could turn these knowledge into dialogues. To bring it to fruition, we propose \da: a \textbf{Plan}ning-based \textbf{D}ata \textbf{A}ugmentation approach that generates synthetic dialogues based on the plans derived from the knowledge bases.}
%synthetically generates a large number of dialogue data shortly. }


\textcolor{blue}{In this paper, we focus on an emerging and challenging troubleshooting task, grounded on flowchart knowledge base, where the agent must identify a problem by asking users a series of questions according to the given flowchart,
as shown in Figure~\ref{fig:intro}.
%each dialogue is grounded on a selected path in flowchart. 
However, as the number of potential paths grows exponentially to the flowchart scales, it's difficult to crowd-source ample dialogue instances that covers all paths. In fact, even the popular \textit{FloDial}~\cite{flowchart2021emnlp} benchmark
%the largest \FTDs benchmark, 
only provides 150 dialogues which cover 65\% of paths in each flowchart on average. }


%collecting sufficient dialogues that cover all potential paths in flowchart is difficult, as the number of paths grows exponentially to the flowchart scales, resulting in a tremendous cost for dialogue annotation.

%Covering all of these paths is difficult because annotating these dialogues is expensive and the number of sub-paths grows exponentially to the flowchart scales. In fact, 
%as shown in Figure~\ref{fig:stat}, \textit{FloDial}, the largest \FTDs benchmark, only provides 1,789 dialogues and covers 
%65\% of the flowcharts sub-paths on average.  

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{images/stat_new.pdf}
%     \caption{Statistics on the percentage (\%) of (un)covered paths in the \textit{FloDial}. In total, more than 35\% of paths are not covered by the dialogue instances in \emph{FloDial}.}
%     \label{fig:stat}
%     \vspace*{-3mm}
% \end{figure}

\textcolor{blue}{The goal of \da is to generate diverse synthetic data by automatically transforming the concise flowchart into dialogues.}  
%Although a selected flowchart path can be regarded an exquisite and logical plan to synthesis dialogue directly, it might generate frustrating and tedious conversations (\eg\ only consist a series of QA). Therefore, \da incorporates dialogue acts  as important features. } 
Specifically, \da takes as input a path in the underlying flowchart and generates a dialogue session consisting of dialogue acts, content, and utterances. It employs a variational framework based on BART pre-trained model~\cite{lewis-etal-2020-bart}, and devises a hierarchical planning strategy which includes \textit{global} and \textit{local} latent planning variables. The \textit{global} latent variable is responsible for modeling the dialogue acts between the the dialogue turns, providing a high-level sketch. 
%To be able to model these global variables, we manually label the dialogue acts for the utterances in the \textit{FloDial} dataset.
For sentence realization, we utilize the \textit{local} latent variable to control the diversity of these synthetic dialogues.




%\emph{Data Augmentation} (DA) is a promising direction to tackle this scarce data issue. DA algorithms aim to effectively extend the existing training instances to improve the performance of downstream tasks. However, many existing DA algorithms, such as EDA~\citep{wei-zou-2019-eda} and back-translation~\citep{zhang-zong-2016-exploiting}, only change the surface tokens of existing training data and retain their semantic meaning. As a result, they cannot produce synthetic data grounding on different flowchart paths. In contrast, \emph{generative data augmentation algorithms}~\citep{DBLP:conf/aaai/Anaby-TavorCGKK20,wang-etal-2022-promda} based on generic pre-trained language models (e.g., GPT-2~\citep{radford2019language}, 
%T5~\citep{10.5555/3455716.3455856}, 
%BART~\citep{lewis-etal-2020-bart}) can potentially generate \emph{brand-new} synthetic data based on different flowchart paths. However, despite being able to produce fluent and natural-looking sentences, these methods are only designed to tackle NLU tasks (e.g., intent detection) and only conditioned on simple input information (e.g., single output labels). They fall short in incorporating appropriate dialogue specific features (e.g., dialogue acts and flowchart information).



%To overcome these limitations, in this paper, we focus on developing \emph{generative data augmentation algorithms} for \FTDs. Our goal is to produce \emph{diverse} synthetic dialogues closely grounded with different floachart paths. \emph{To this end,} we propose a {\em Variational Data Augmentation} ({\em VarDA}\/) approach for generating. \emph{VarDA} takes as input a path in the underlying flowchart and generates a dialogue session consisting of dialogue acts, content, and utterances. It
%employs a hierarchical planning strategy which includes \textit{global} and \textit{local} latent planning variables. 
%The \textit{global} latent variable is responsible for modeling the dialogue acts between the the dialogue turns, providing a high-level sketch. 
%To be able to model these global variables, we manually label the dialogue acts for the utterances in the \textit{FloDial} dataset. For sentence realization, we utilize the \textit{local} latent variable to control the diversity of these synthetic dialogues.

We conduct our experiments on the \textit{FloDial} benchmark. Experiment results show that the retrieval and generative models trained on the synthetic dialogues produced by \da achieve better performance in the flowchart path retrieval and response generation downstream tasks, in particularly on the \textit{Out-of-Domain} settings. We also conduct ablation study to show the effectiveness of our proposed \textit{global} and \textit{local} latent planning variables. We then conduct \textit{extrinsic} evaluation to examine the quality of the synthetic dialogues produced by \da and find that they outperform strong baseline models in term of diversity and faithfulness. We finally showcase our generated synthetic dialogues for covered and uncovered paths.


==> introduction_yufei.tex <==
\section{Introduction}
Task-oriented dialogue (TOD) systems  are designed to complete specific tasks through conversation with human, e.g.,  ticket booking~\cite{wen2016network} or problem diagnosis~\cite{boye2007dialogue,flowchart2021emnlp}. To achieve their goals, TOD systems usually require large amount of dialogues grounded to specific domain knowledge from external databases or online APIs. While dialogue corpora are abundant on the Internet, they mostly focus on personal anecdotes and subjective opinions, and is thus unsuitable for
TOD systems, which desire responses with domain knowledge. Directly crowd-sourcing dialogues can also be challenging: crowd-workers are rarely domains experts with massive task-specific knowledge and tend to provide shallow dialogue content~\citep{li-etal-2022-ditch}. In this paper, we focus on an emerging and challenging type of TOD systems,  troubleshooting dialogue grounded on flowchart knowledge base. As shown in Figure~\ref{fig:intro}, in this task, the agent must identify a problem by asking users a series of questions according to the given flowchart. Flowchart troubleshooting dialogue also suffers from data sparsity issue discussed above. Furthermore, the number of potential paths grows exponentially to the flowchart scales, making it challenging to collect dialogues that covers all paths. Even the \textit{FloDial}~\cite{flowchart2021emnlp} benchmark only provides 150 dialogues which cover 65\% of paths in each flowchart on average. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.99\linewidth]{images/flow_intro_acl2023.pdf}
    \caption{A sample flowchart-grounded troubleshooting dialogue. Agent follows the path of a flowchart to help user diagnose  problems.}
    \label{fig:intro}
\end{figure}

To overcome this challenge, some recent work utilize data augmentation algorithm to generate synthetic data. However, existing data augmentation approaches, \eg\ back-translation~\citep{zhang-zong-2016-exploiting}, EDA~\citep{wei-zou-2019-eda} and PARG~\cite{gao2020paraphrase}, only replace the surface tokens or paraphrase sentences, and retain their semantic meaning. \textcolor{blue}{As a result, these methods are limited to produce synthetic data conditioned on previously covered knowledge. The uncovered knowledge are still missing from the generated synthetic data.} Observing that high-quality knowledge base, \eg\ structured flowchart, are abundant, the ideal solution is to directly generate \emph{brand-new} synthetic dialogues from these uncovered knowledge \eg\ flowchart paths.

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{images/stat_new.pdf}
%     \caption{Statistics on the percentage (\%) of (un)covered paths in the \textit{FloDial}. In total, more than 35\% of paths are not covered by the dialogue instances in \emph{FloDial}.}
%     \label{fig:stat}
%     \vspace*{-3mm}
% \end{figure}

To bring it to fruition, in this paper, we propose \da: a \textbf{Plan}ning-based \textbf{D}ata \textbf{A}ugmentation approach that generates synthetic dialogues \textcolor{blue}{using the uncovered flowchart paths.} The goal of \da is to generate diverse synthetic data by automatically transforming the concise flowchart into dialogues. Specifically, \da takes as input a path extracted from the underlying flowchart and generates a dialogue session consisting of dialogue acts, and utterances. It employs a variational framework based on BART pre-trained model~\cite{lewis-etal-2020-bart}, and devises a hierarchical planning strategy which includes \textit{global} and \textit{local} latent planning variables. The \textit{global} latent variable is responsible for modeling the dialogue acts between the the dialogue turns, providing a high-level sketch, while the \textit{local} latent variable controls the diversity of local utterance generation.

We conduct our experiments on the \textit{FloDial} benchmark. Experiment results show that the retrieval and generative models trained on the synthetic dialogues produced by \da achieve better performance in the flowchart path retrieval and response generation downstream tasks, in particularly on the \textit{Out-of-Domain} settings. We also conduct ablation study to show the effectiveness of our proposed \textit{global} and \textit{local} latent planning variables. We then conduct \textit{extrinsic} evaluation to examine the quality of the synthetic dialogues produced by \da and find that they outperform strong baseline models in term of diversity and faithfulness. We finally showcase our generated synthetic dialogues for covered and uncovered paths.


==> limitations.tex <==
\section*{Limitations}
%%We discuss the potential limitations of our %%work in the section.
Due to limited access to open-source datasets for FTD systems, we have conducted our experiments only on the \textit{FloDial} dataset. In  future, it will be beneficial to evaluate our method as new datasets become available.  As a future work direction, it would be interesting to devise effective and efficient evaluation methods for synthetically generated dialogue data.
%%provide the results of human evaluation in next version or the author response period.

==> method.tex <==
\section{Pseudo Dialogue Synthesis }
\subsection{Task Formulation}
Given a sub-path $\textbf{x} = \{{x}_1, {x}_2, \ldots, {x}_n\}$ in a flowchart as input, where each $x_i$ is a question-answer pair in the flowchart (e.g., ``starter cranks? No'' in Figure~\ref{fig:intro}) or a problem statement, our task is to generate a long and diverse synthetic pseudo conversation $\textbf{y} = \{{y}_1, {y}_2, \ldots, {y}_m\}$ where $\textbf{y}_i$ is the $i$-th utterance in this dialogue, and a sequence of corresponding dialogue acts $\textbf{a} = \{{a}_1, {a}_2, \ldots, {a}_m\}$.
\reza{what's the relation between $n$ and $m$? why the dialogue acts 'a' are boldface here, but not in the rest of the section? why 'x' is bold here but not bold in the rest of the section?}

% Given input data $x = \{x_1, x_2,...,x_n\}$ where each $x_i$ can be an short prompt sentence or instruction (e.g., flowchart node description), our task is to generate a long and diverse pseudo dialogue content $y = \{y_1,y_2,...,y_m\}$ that $y_i$ is the $i$-th utterance of generative pseudo dialogue, and a sequence of dialogue act (DA) $a = \{a_1, a_2,...,a_m\}$. The generative pseudo dialogue content should follow the plan and order of input prompt sentence. For each of the $y_i$ and its corresponding dialogue act $a_i$, it might contains 1 to 3 sub-sentences and sub-dialogue acts, e.g. $y_i = <y_i^1,...,y_i^j>$ and $a_i = <a_i^1,...,a_i^j>$, while $j \in [1,3]$.

% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.95\linewidth]{images/overall.pdf}
% \label{screenshot}
% \vspace{-3mm}
% \caption{Overall graphical model of our proposed model.}
% \label{fig:overall}
% \end{figure}

\begin{figure*}
\centering
\includegraphics[width=1.0\linewidth]{images/explanation.pdf}
\label{screenshot}
\vspace{-3mm}
\caption{Detailed architecture of the VarDA model.}
\label{fig:framework}
\end{figure*}

\subsection{Approach Overview}
Our approach devises a variational data augmentation model (VarDA) with hierarchical planning strategy. It contains two planning latent variables: global planning latent variable $\mathbf{z}^a$ and local planning latent variable $\mathbf{z}^y$. The global planning latent variable $\mathbf{z}^a$ is responsible for modeling the dialogue act transition process (e.g., inform, Yes-No-question, clarify), also known as high-level sketch. The local planning latent variable $\mathbf{z}_y$ is responsible for generating lexically diverse utterances to realize dialogue acts, also known as low-level realization.

The global planning decoder takes $\mathbf{z}^a$ as initial input, and at time step $t$, it decodes a dialogue act $a_t$. Then, the utterance generator produces corresponding sentence, considering both the input $x_t$, the dialogue act $a_t$, and local latent variable $\mathbf{z}^a$ (Figure~\ref{fig:framework}). The planning process decomposes the long dialogue synthetic process into a series of context-dependent sentence generation sub-tasks. It could manage the generation process in a precise way, depending on the hierarchical variational latent structures. 

%\subsection{Input Representation}
% We use the pre-trained model BART~\cite{lewis2020bart} to initialize our representation for input data $x = \{x_1, x_2,...,x_n\}$ where each $x_i$ at the encoder side, and $y$ at the decoder side.
% The initial representation of ${\bf x}$ is the sum of word, position and turn-level embeddings:
% \begin{align*}
%     \mathbf{e}_{\bf x} &= {\rm WE}({\bf x}) + {\rm PE}({\bf x}) + {\rm TE}({\bf x}), \\
%      \mathbf{H}_{\bf x} &= {\rm BART}_{large}(\mathbf{e}_{\bf x}), \mathbf{h}_{\bf x} = \mathrm{Avgpool}(\mathbf{H}_{\bf x}),
% \end{align*}
% where $\mathbf{e}_{\bf c}$ and $\mathbf{h}_{\bf c}$ are the initial representation and hidden representation after BERT of dialogue context. ${\rm WE}(\cdot)$, ${\rm PE}(\cdot)$ and ${\rm TE}(\cdot)$ refer to the word-level, position-level and turn-level embeddings respectively. ${\rm Avepool(\cdot)}$ is the average pooling operation~\cite{cer2018universal}. 

% % Take pre-trained model as intial representation: aT-2/BART. (Details omitted temporarily for further development)

\subsection{Global Planning with Dialogue Act}
Dialogue acts describe the function of dialogue utterance, and reflect a user's intent. Therefore, dialogue acts play an important role in the generation of synthetic pseudo dialogues. %%which can be regarded as high-level sketch for detailed utterance generation.
As mentioned above, we employ a global planning process to generate a sequence of dialogue acts.
Prior to global planning, we use the pre-trained model BART~\cite{lewis2020bart} to initialize our representation of the input data $x = \{x_1, x_2,...,x_n\}$. The hidden representation of input data is formulated as
$\mathbf{h}^{x} = \{\mathbf{h}^{x}_{1},...,\mathbf{h}^{x}_{n}\}$.
\reza{do you mean $\mathbf{h}^x$ to be the 'collection' of $\mathbf{h}_i^x$? In the rest of this section, you have used $\mathbf{h}^x$ in the conditioning context of the probabilities, so not sure whether it should be a sequence of vectors or just a vector? Also, each $x_i$ is a 'sequence' of words (corresponding to the text in a node together with the user response on the outgoing edge), right? then when $x_i$ is fed to BERT, in fact a sequence is fed into BERT?}

The global planning process can be formulated as follows:
\begin{align}
    a_t = \text{argmax} P(a_t |a_{<t}, \mathbf{h}^{x}, \mathbf{z}^a)
\end{align}
where $a = \{a_1,...a_m\}$ is a sequence of dialogue acts.
The global planning latent variable $\mathbf{z}_a$ is assumed to follow the Gaussian distribution~\cite{kingma2014auto}, and the prior and posterior distributions are formulated by $p_\theta (\mathbf{z}_a | \mathbf{h}^{x})$ and $q_\phi (\mathbf{z}_a | \mathbf{h}^{x}, \mathbf{h}^{y})$ respectively. 
where the parameters ${\bf \sigma}$ and ${\bf \mu}$ are estimated by:
\begin{align*}
    & \bm{\mu}^p = \text{MLP}^p_\theta({\mathbf{h}^{x}}),  \bm{\sigma}^p = \text{softplus}(\text{MLP}^p_\theta(\mathbf{h}^{x})), \\
    & \bm{\mu}^q = \text{MLP}^q_\phi([{\mathbf{h}^{x},\mathbf{h}^{y}]}),  \bm{\sigma}^q = \text{softplus}(\text{MLP}^q_\phi([\mathbf{h}^{x}, \mathbf{h}^{y}])),
\end{align*}
where ${\rm MLP}(\cdot)$ denotes multiple layer perception, and ${\rm softplus(\cdot)}$ is a smooth approximation to ReLU, which ensures positiveness.
We give the Evidence Lower Bound (ELBO) as follows:
\begin{eqnarray*}
    \mathcal{L}_{\mathrm{global}} & = & -KL(q_\phi({\bf z}^{\bf a}|{\bf h}^{x}, {\bf h}^{y})||p_\theta({\bf z}^{\bf a}|{\bf h}^{x})) \\
    & & + \mathbb{E}_{{\bf z}^{\bf a} \sim q_\phi}[\log p_{\theta}({a} |{\bf z}^{\bf a},\textbf{h}^{x})]
\end{eqnarray*}
where $D_{KL}(\cdot |\cdot)$ refers to Kullback-Leibler divergence~\cite{kullback1951information}.

At time step $t$, the global planning process decodes each of the $a_{t}$ in $a$ by calculating the probability $P(a_{t} | a_{<t}, x, z_a)$. The training loss function at time step $t$ is formulated as:
\begin{eqnarray*}
  \lefteqn{-\log P(a_{t}=\hat{a}_{t} | a_{<t}, {\bf z}^{\bf a},\textbf{h}^{x})} \\
     &= & - \sum_{a_{t} = \hat{a}_{t}} \log P(a_{t}) 
     - \sum_{a_{t} \neq \hat{a}_{t}} \log(1 - P(a_{t})) 
\end{eqnarray*}

\subsection{Local Planning for Utterance Generation}
The local sentence planning module aims to generate diverse dialogue utterances $y = \{y_1,y_2,...,y_m\}$ that are faithful to the flowchart. For each utterance $y_i$, the utterance decoder considers the information corresponding to a node in the flowchart $x_i$, the corresponding dialogue act $a_i$ and the local planning variable $z^y$ by computing:
\begin{align}
    y_t = \text{argmax} P (y_t | y_{<t}, \mathbf{h}^{x}, a, \mathbf{z}^y)
\end{align}

The local planning process is similar to the global planning process. The local planning latent variable $z^y$ is assumed to follow the Gaussian distribution $\mathcal{N}({\bf \mu},{\bf \sigma^{2}I})$. and the prior and posterior distributions are formulated by $p_\theta (z^y | y_{<t}, x, a)$ and $q_\phi (z^y |y_{<=t}, x, a)$. The parameters $\theta$ and $\mu$ in this Gaussian distribution are estimated by:\\
$\bm{\mu}^p_{y} = \text{MLP}^p_\theta({\bf h}^{x},{ a},{\bf h}^{y}_{<t}),  \bm{\sigma}^p_{y} = \text{softplus}(\text{MLP}^p_\theta({\bf h}^{x},{ a},{\bf h}^{y}_{<t})),$\\
and the posterior parameters are estimated by:\\
$\bm{\mu}^q_{y} = \text{MLP}^q_\phi({\bf h}^{x},{a},{\bf h}^{y}_{\leq t}),  \bm{\sigma}^q_{y} = \text{softplus}(\text{MLP}^q_\phi({\bf h}^{x},{a},{\bf h}^{y}_{\leq t}).$

The decoder is also initialized by the BART model. It decodes a specific utterance $y_i$ conditioned on $\{ y_{<t}, \mathbf{h}^{x}, a, \mathbf{z}^y\}$. We give the ELBO for local planning as follows:
\begin{eqnarray*}
    \lefteqn{\mathcal{L}_{\mathrm{local}} =}\\
    & & -KL(q_\phi({\bf z}^{\bf y}|{\bf h}^{x},{ a},{\bf h}^{y}_{<t})||p_\theta({\bf z}^{\bf y}|{\bf h}^{x},{ a},{\bf h}^{y}_{\leq t})) \\
    & & +\mathbb{E}_{{\bf z}^{\bf y} \sim q_\phi}[\log p_{\theta}({y}_{t} |y_{<t}, \mathbf{h}^{x}, a, \mathbf{z}^y)].
\end{eqnarray*}

The overall objective to be maximized is the  sum of the ELBOs:
$\mathcal{L}_{\mathrm{all}} = \mathcal{L}_{\mathrm{global}} + \mathcal{L}_{\mathrm{local}}.$













==> method_haolan_v2.tex <==
\section{Planning-based Data Augmentation}
In this section, we first introduce the task formulation in Section~\ref{formulation}. We then describe flowchart path extraction in Section~\ref{pathextract}. We further discuss the general design of our proposed method \da in Section~\ref{generationstory} as well as its important global planning and local planning components in Section~\ref{globalgeneration} and~\ref{localgeneration}, respectively. Figure~\ref{fig:framework} shows the overview of \da.

\subsection{Task Formulation}
\label{formulation}
\textcolor{blue}{The goal of \da is to take a sampled path (selected from a flowchart, which contains multiple paths), and generate a complete dialogue by incorporating flowchart path and dialogue acts.}

\textcolor{blue}{In this paper, we only have access to a handful training set $\gT=\{(\vx,\va,\vy)_i\}_{i=1}^m$ where ${\vx} = \{{x}_1, {x}_2, \ldots, {x}_n\}$ is a flowchart sub-path, $\va = \{a_1,..,a_n\}$ is the sequence of dialogue acts and $\vy = \{{y}_1, {y}_2, \ldots, {y}_n\}$ is the dialogue. Note that $x_i$ is the $i$-th flowchart node in path ${\vx}$. $y_i$ in the $i$-th sub-dialogue consisting of several utterances and each utterance has its own dialogue act. Given a flowchart sub-path $\vx$, our proposed \emph{Data Augmentation} method \da generates synthetic dialogue acts $\hat{\va}$ and dialogues $\hat{\vy}$ and produces the final synthetic dataset $\gT_{Syn}=\{(\vx, \hat{\va},\hat{\vy})_i\}_{i=1}^n$ where $n$ could be much larger than $m$ (e.g., 10x). Our goal is that the downstream retrieval and generative dialogue models trained using $\gT \cup \gT_{Syn}$ outperform the ones only trained using $\gT$. }


% each $x_i$ is a question-answer pair in the flowchart (\eg\ ``starter cranks? No'' in Figure~\ref{fig:intro}) or a problem statement phrase (\eg\ car won't start)


% {We are given} a sub-path  in a flowchart as input, where  .
% %
% Our task is to generate a diverse synthetic pseudo conversation ${\vy} = \{{y}_1, {y}_2, \ldots, {y}_n\}$ where ${y}_i$ is the $i$-th turn in this dialogue.
% %
% We assume that  $y_i$ in the $i$-th turn consists of several utterances $\{y_{i,j}\}_{j=1}^{|y_i|}$ where each utterance has its own dialogue act $a_{i,j}$. As such, {we can capture} the multiple dialogue acts setting in a single turn. We denote the sequence of {dialogue acts by} $\va = \{a_1,..,a_n\}$ where $a_i = \{a_{i,j}\}_{j=1}^{|a_i|}$, {and $a_{i,j}$ is the dialogue act of corresponding utterance $y_{i,j}$.}  


\begin{figure*}
\centering
\includegraphics[width=1\linewidth]{images/method_acl2023_yufei.pdf}
\label{screenshot}
\vspace{-3mm}
\caption{Detailed architecture of the PlanDA model.}
\label{fig:framework}
\end{figure*}

\subsection{Flowchart Path Extraction}
\label{pathextract}
\textcolor{red}{As shown in Figure~\ref{fig:intro}, the flowcharts used in this paper consist of decision nodes and action nodes. The decision nodes include question and they are connected with others by the user responses (e.g., Yes, No). The action nodes are at the bottom of the flowcharts indicating appropriate actions. For training, we directly extract the flowchart paths in the training data. For syntactic data generation, to ensure the full coverage for the flowchart paths, we extract the flowchart paths by the \emph{Depth-First-Search} from the top decision nodes until and bottom action nodes. The resulting flowchart paths are then used as the inputs for \da.}  




\subsection{Overview of \da}
\label{generationstory}
\textcolor{red}{Given the extracted flowchart paths, \da is designed to generate diverse and high-quality synthetic dialogues. Although the input flowchart paths include textual questions, user responses and final actions, only conditioning on these information could result in frustrating and tedious conversations (\eg\ only consist a series of QA). Thus, we propose to use dialogue acts, which describe high-level information (e.g., inform, clarification) about a single utterance, as a planning variable to enrich the generation process.} Specifically, we equip \da  with {a} hierarchical planning strategy. It contains two planning latent variables: global planning latent variable $\mathbf{z}^a_i$ and local planning latent variable $\mathbf{z}^y_{i,j}$. The global planning latent variable $\mathbf{z}^a_i$ is responsible for modeling the {dialogue act transition process \emph{{over the turns}}, %(e.g., inform, yes-no-question, clarification), 
also known as high-level sketch}. The local planning latent variable $\mathbf{z}^y_{i,j}$ is responsible for generating lexically diverse utterances to realize dialogue acts, also known as low-level realization.


%At inference stage, PlanDA model will generate the dialogue context step by step. 
Specifically, we perform the following steps to generate the utterances corresponding to $x_i$.  
%
We start by sampling the global latent variable $\vz^{a}_i \sim p^{\vz^a}_{\theta}(. | x_i)$.
%where $\vh_i^{x}$ is the representation of $x_i$. 
We then sample the $y_{i,j}$ as follows:
\begin{itemize}
\itemsep0em
    \item Sample the  dialogue act:\\  $a_{i,j}~\sim~p^{a}_{\theta}(. | a_{i,j-1}, x_i,\vz^a_i)$
    \item Sample the local latent variable:\\
$\vz^{y}_{i,j}~\sim~p^{\vz^y}_{\theta}(. | x_i, a_{i,j})$   
\item Sample the utterance:\\
 $y_{i,j}~\sim~p^y_{\theta}(.|y_{i,j-1}, x_i, a_{i,j}, \vz_{i,j}^y)$
\end{itemize}

As the $\vz$ variables are continuous latent variables, the probability of generating a conversation and the corresponding dialogue acts given the flowchart path can be written as follows:
\begin{eqnarray}
\label{eqn:probgen}
\lefteqn{p_{\theta}(\vy,\va|\vx) = \prod_i  \int d(\vz_i^a)  p_{\theta}^{\vz^a}(\vz_i^a|x_i)}  \\  
    &&  \times \prod_j \int d(\vz_{i,j}^y)    p_{\theta}^a(a_{i,j}|a_{i,j-1},x_i, \vz_i^a) \nonumber \\ 
    && \times p_{\theta}^{\vz^y}(\vz_{i,j}^y|x_i,a_{i,j}) p^y_{\theta}(y_{i,j}|y_{i,j-1}, x_i, a_{i,j}, \vz_{i,j}^y) \nonumber
\end{eqnarray}

Next, we describe how we operationalise the probability terms in Equation~\ref{eqn:probgen} using neural architectures, and how we learn the model parameters using the variational approach to overcome the challenges of integration over the latent variables. 

%The global planning decoder takes $\mathbf{z}^a$ as initial input, and at time step $t$, it decodes a dialogue act $a_t$. Then, the utterance generator produces corresponding sentence, considering both the input $x_t$, the dialogue act $a_t$, and local latent variable $\mathbf{z}^y$ (Figure~\ref{fig:framework}). The planning process decomposes the long dialogue synthetic process into a series of context-dependent sentence generation sub-tasks. 
% It could manage the generation process in a precise way, depending on the hierarchical variational latent structures. 

%At decoder side, ground truth $y$ is encoded in the similar way.

%The hidden representation of input data is formulated as $\mathbf{h}_{x} = \{\mathbf{h}_{{x}_{1}},...,\mathbf{h}_{{x}_{n}}\}$.
%For each representation of ${\bf h}_{x_i}$, it is embedded through BART model following with a Average pooling operation~\cite{cer2018universal}: $\mathbf{h}_{x_i} = \text{Avgpool}({\rm BART}(x_i))$. At decoder side, ground truth $y$ is encoded in the similar way.

% % Take pre-trained model as intial representation: aT-2/BART. (Details omitted temporarily for further development)

\subsection{Global Planning with Dialogue Acts}
\label{globalgeneration}
Dialogue acts describe the basic function of a dialogue utterance (\eg\ inform, clarification), and reflect user intents~\cite{stolcke2000dialogue,bunt2011semantics}. Synthetic dialogue generation task is not only about sentence generation, but also incorporating dialogue-specific features. Dialogue acts, as one of representatives in dialogue features,  play an important role in the generation of synthetic pseudo dialogues. In the \textit{FloDial} dataset, for each utterance $y_{i,j}$, there is a corresponding dialogue act tag.
%%which can be regarded as high-level sketch for detailed utterance generation.

We employ a global planning process to generate a sequence of dialogue acts.
% Prior to global planning, we use the pre-trained model BART~\cite{lewis2020bart} to initialize our representation of the input data $x = \{x_1, x_2,...,x_n\}$. The hidden representation of input data is formulated as
% $\mathbf{h}_{x} = \{\mathbf{h}_{{x}_{1}},...,\mathbf{h}_{{x}_{n}}\}$.
% \reza{do you mean $\mathbf{h}^x$ to be the 'collection' of $\mathbf{h}_i^x$? In the rest of this section, you have used $\mathbf{h}^x$ in the conditioning context of the probabilities, so not sure whether it should be a sequence of vectors or just a vector? Also, each $x_i$ is a 'sequence' of words (corresponding to the text in a node together with the user response on the outgoing edge), right? then when $x_i$ is fed to BERT, in fact a sequence is fed into BERT?}
%
%The global planning process can be formulated as follows:
%\begin{align*}
%    a_t = \text{argmax} P(a_t |a_{<t}, \mathbf{h}^{x}, \mathbf{z}^a)
%\end{align*}
%where $a = \{a_1,...a_n\}$ is a sequence of dialogue acts. 
%
Specifically, we inject stochasticity to this process using a continuous latent variable in each dialogue turn
%To construct the global planning latent variable 
$\vz^a_i$, which is assumed to follow the isotropic Gaussian distribution~\cite{kingma2014auto}. Given Gaussian  prior distributions 
$p_\theta^{\vz^a} (\vz^a_i | x_i)$, 
we propose to approximate the  posterior distribution $q_\phi (\vz^a_i  | x_i, y_i)$ using Gaussians in the  training phase.
% The global planning latent variable $\mathbf{z}^a$ is assumed to follow the Gaussian distribution~\cite{kingma2014auto}, and the prior and posterior distributions are formulated by $p_\theta (\mathbf{z}_a | \mathbf{h}^{x})$ and $q_\phi (\mathbf{z}_a | \mathbf{h}^{x}, \mathbf{h}^{y})$ respectively. 
The parameters $\bm{\mu}^{p}_{a}$, $\bm{\sigma}^{p}_{a}$,  $\bm{\mu}^{q}_{a}$ and $\bm{\sigma}^{q}_{a}$ of the prior and posterior distributions are parameterised with neural networks as follows:
\begin{align*}
    \bm{\mu}^p_{a} &= \text{MLP}^p_\theta({\vh^{x}_i}), \\
    \bm{\sigma}^p_{a} &= \text{softplus}(\text{MLP}^p_\theta(\vh^{x}_i)), \\
    \bm{\mu}^q_{a} &= \text{MLP}^q_\phi([{\vh^{x}_i,\vh^{y}_i]}), \\
    \bm{\sigma}^q_{a} &= \text{softplus}(\text{MLP}^q_\phi([\vh^{x}_i,\vh^{y}_i])), \\
\end{align*}
where ${\rm MLP}(\cdot)$ denotes a multi-layer perceptron, and ${\rm softplus(\cdot)}$ is a smooth approximation to ReLU, which ensures positiveness.
%
Each $x_i$ is fed into the encoder of the BART model ~\cite{lewis2020bart}, and followed by an average pooling operation~\cite{cer2018universal} to get its representation: $\vh_i^{x} = \text{AvgPool}({\rm BART}(x_i))$. 
%
We use a similar process to encode each utterance $y_{i,j}$ in the $i$-th turn, and then apply average pooling over the resultant representations in this turn to get $\vh_i^y$.

The Evidence Lower Bound (ELBO) is computed as follows:
%\footnote{See the derivation  in the Appendix.}, 
%\vspace*{-2mm}
\begin{eqnarray*}
  \lefteqn{\mathcal{L}_{\mathrm{global}}  =  -D_{KL}(q_\phi({\vz}^{a}_i|{x}_i, {y}_i)||p_\theta^{\vz^a}({\vz}^{a}_i|{x}_i))} \\
    & & + \mathbb{E}_{{\vz}^{a}_i \sim q_\phi}[\sum_j \log p_{\theta}^a({a_{i,j}} |a_{i,j-1},{\vz}^{ a}_i,{x}_i)]
   % \vspace*{-2mm}
\end{eqnarray*}
where $D_{KL}(\cdot |\cdot)$ refers to Kullback-Leibler divergence~\cite{kullback1951information}.
%
The dialogue act probability function $p_{\theta}^a(a_{i,j} |a_{i,j-1}, {\vz}^{ a}_i,\vh^{x}_i)$ is a 2-layer MLP with the softmax on top. 
%

%At time step $t$, A sample of ${\bf z}^{a}$ using the reparametrization
%trick~\cite{kingma2014auto} is then fed into the global planning decoder. Each $a_{t}$ is decoded by calculating the probability $P(a_{t} | a_{<t}, {\bf h}_{x_t}, {\bf z}^{a})$. The training loss function at time step $t$ is formulated as:
%\begin{eqnarray*}
%  \lefteqn{-\log P(a_{t}=\hat{a}_{t} | a_{<t}, \textbf{h}^{x},{\bf z}^{\bf a})} \\
%     &= & - \sum_{a_{t} = \hat{a}_{t}} \log P(a_{t}) 
%     - \sum_{a_{t} \neq \hat{a}_{t}} \log(1 - P(a_{t})).
%\end{eqnarray*}

\subsection{Local Planning for Utterance Generation}
\label{localgeneration}
The local sentence planning module aims to generate lexically diverse dialogue utterances $\vy = \{y_1,y_2,...,y_n\}$ that are faithful to the flowchart. For the $j$-th utterance in the $i$-th turn $y_{i,j}$, the utterance decoder considers the information corresponding to the node in the flowchart $x_i$, the corresponding dialogue act $a_{i,j}$ and the local planning variable $\vz^y_{i,j}$ by sampling the utterance from $p^y_{\theta}(.|y_{i,j-1}, x_i, a_{i,j}, \vz_{i,j}^y)$.
%\begin{align*}
%    y_t = \text{argmax} P (y_t | y_{<t}, \mathbf{h}^{x}, \mathbf{h}^{a}, \mathbf{z}^y),
%\end{align*}
%
We provide the representation of the conditioning context to the BART encoder, and generate the utterance via the decoder. 
%
We simply concatenate (non-linear transformation) the following: $\vh_{i,j-1}^y, \vz_{i,j}^y, \vh_i^x$ and $ \vh^a_{i,j}$, which is the embedding of the dialogue act $a_{i,j}$. The BART decoder then attends to these  vectors to generate the output utterance.  

The construction of local planning latent variable ${\vz}^{y}_{i,j}$ is similar to that of the global latent variable. We assume that it follows the Gaussian distribution.
%cal plannThe loing process is similar to the global planning process. The local planning latent variable $z^y$ is assumed to follow the Gaussian distribution $\mathcal{N}({\bf \mu},{\bf \sigma^{2}I})$. and 
The prior and posterior distributions are formulated by $
p_\theta^{\vz^y} (\vz^y_{i,j} | x_i, a_{i,j})$ and $q_\phi (\vz^y_{i,j} | x_i, a_{i,j}, y_{i,j})$, and they are parameterised as follows:
{
\begin{eqnarray*}
\bm{\mu}^p_{y} & = & \text{MLP}^p_\theta({\vh}^{x}_i,\vh^a_{i,j}), \\
\bm{\sigma}^p_{y} & = &\text{softplus}(\text{MLP}^p_\theta({\vh}^{x}_i,\vh^a_{i,j})\\
\bm{\mu}^q_{y} & = & \text{MLP}^q_\phi({\vh}^{x}_i,\vh^a_{i,j},\vh^y_{i,j}), \\ \bm{\sigma}^q_{y}
& = & \text{softplus}(\text{MLP}^q_\phi({\vh}^{x}_i,\vh^a_{i,j},\vh^y_{i,j}).
\end{eqnarray*}
}

%The decoder for utterance generation is also initialized by the BART model. For the $j$-th word in $y_t$ utterance, the word $y_t^{j}$ is decoded on the condition $\{y_t^{\textless j}, y_{<t}, \mathbf{h}^{x}, a, \mathbf{z}^y\}$. 
The ELBO for local planning is:
\vspace*{-2mm}\begin{eqnarray*}
    \lefteqn{\mathcal{L}_{\mathrm{local}} =}\\
    & & \!\!\!-D_{KL}(q_\phi({\vz}^{y}_{i,j}|{x}_i,a_{i,j}, y_{i,j})||p_\theta^{\vz^y}({\vz}^{y}_{i,j}|{x}_i,a_{i,j})) \\
    & & \!\!\!+\mathbb{E}_{{\vz}^{y}_{i,j} \sim q_\phi}[\log p_{\theta}({y}_{i,j} |y_{i,j-1}, x_i, a_{i,j}, \vz^y_{i,j})].
\end{eqnarray*}

The overall training objective to be optimised is the  sum of the ELBOs:
$\mathcal{L}_{\mathrm{all}} = \mathcal{L}_{\mathrm{global}} + \mathcal{L}_{\mathrm{local}}.$
We use the reparametrization
trick in~\cite{kingma2014auto} to optimise  the training objective. 

==> method_new.tex <==
\section{Variational DA for \FTDs}

\subsection{Task Formulation}
\label{formulation}
{We are given} a sub-path ${\vx} = \{{x}_1, {x}_2, \ldots, {x}_n\}$ in a flowchart as input, where each $x_i$ is a question-answer pair in the flowchart (\eg\ ``starter cranks? No'' in Figure~\ref{fig:intro}) or a problem statement phrase (\eg\ car won't start) .
%
Our task is to generate a diverse synthetic pseudo conversation ${\vy} = \{{y}_1, {y}_2, \ldots, {y}_n\}$ where ${y}_i$ is the $i$-th turn in this dialogue.
%
We assume that  $y_i$ in the $i$-th turn consists of several utterances $\{y_{i,j}\}_{j=1}^{|y_i|}$ where each utterance has its own dialogue act $a_{i,j}$. As such, {we can capture} the multiple dialogue acts setting in a single turn. We denote the sequence of {dialogue acts by} $\va = \{a_1,..,a_n\}$ where $a_i = \{a_{i,j}\}_{j=1}^{|a_i|}$, {and $a_{i,j}$ is the dialogue act of corresponding utterance $y_{i,j}$.}  
%
We assume access to a training dataset consisting of $(\vx,\va,\vy)$ tuples. 
% \reza{what's the relation between $n$ and $m$? why the dialogue acts 'a' are boldface here, but not in the rest of the section? why 'x' is bold here but not bold in the rest of the section?}
% \haolan{To avoid misunderstanding, I just keep the same number of x, y, a. In our implementation, the input is actually ($x_1, x_2, x_2, x_3, x_3, ....$)}

% Given input data $x = \{x_1, x_2,...,x_n\}$ where each $x_i$ can be an short prompt sentence or instruction (e.g., flowchart node description), our task is to generate a long and diverse pseudo dialogue content $y = \{y_1,y_2,...,y_m\}$ that $y_i$ is the $i$-th utterance of generative pseudo dialogue, and a sequence of dialogue act (DA) $a = \{a_1, a_2,...,a_m\}$. The generative pseudo dialogue content should follow the plan and order of input prompt sentence. For each of the $y_i$ and its corresponding dialogue act $a_i$, it might contains 1 to 3 sub-sentences and sub-dialogue acts, e.g. $y_i = <y_i^1,...,y_i^j>$ and $a_i = <a_i^1,...,a_i^j>$, while $j \in [1,3]$.

% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.95\linewidth]{images/overall.pdf}
% \label{screenshot}
% \vspace{-3mm}
% \caption{Overall graphical model of our proposed model.}
% \label{fig:overall}
% \end{figure}

\begin{figure*}
\centering
\includegraphics[width=1\linewidth]{images/EACL_framework.pdf}
\label{screenshot}
\vspace{-3mm}
\caption{Detailed architecture of the VarDA model.}
\label{fig:framework}
\end{figure*}

\subsection{A Generative Story}
\label{generationstory}
%\subsection{Approach Overview}
Our approach devises a variational data augmentation model (VarDA) with {a} hierarchical planning strategy. It contains two planning latent variables: global planning latent variable $\mathbf{z}^a_i$ and local planning latent variable $\mathbf{z}^y_{i,j}$. The global planning latent variable $\mathbf{z}^a_i$ is responsible for modeling the {dialogue act transition process \emph{{over the turns}}, %(e.g., inform, yes-no-question, clarification), 
also known as high-level sketch}. The local planning latent variable $\mathbf{z}^y_{i,j}$ is responsible for generating lexically diverse utterances to realize dialogue acts, also known as low-level realization.


%At inference stage, VarDA model will generate the dialogue context step by step. 
Specifically, we perform the following steps to generate the utterances corresponding to $x_i$.  
%
We start by sampling the global latent variable $\vz^{a}_i \sim p^{\vz^a}_{\theta}(. | x_i)$.
%where $\vh_i^{x}$ is the representation of $x_i$. 
We then sample the $y_{i,j}$ as follows:
\begin{itemize}
\itemsep0em
    \item Sample the  dialogue act:\\  $a_{i,j}~\sim~p^{a}_{\theta}(. | a_{i,j-1}, x_i,\vz^a_i)$
    \item Sample the local latent variable:\\
$\vz^{y}_{i,j}~\sim~p^{\vz^y}_{\theta}(. | x_i, a_{i,j})$   
\item Sample the utterance:\\
 $y_{i,j}~\sim~p^y_{\theta}(.|y_{i,j-1}, x_i, a_{i,j}, \vz_{i,j}^y)$
\end{itemize}

As the $\vz$ variables are continuous latent variables, the probability of generating a conversation and the corresponding dialogue acts given the flowchart path can be written as follows:
\begin{eqnarray}
\label{eqn:probgen}
\lefteqn{p_{\theta}(\vy,\va|\vx) = \prod_i  \int d(\vz_i^a)  p_{\theta}^{\vz^a}(\vz_i^a|x_i)}  \\  
    &&  \times \prod_j \int d(\vz_{i,j}^y)    p_{\theta}^a(a_{i,j}|a_{i,j-1},x_i, \vz_i^a) \nonumber \\ 
    && \times p_{\theta}^{\vz^y}(\vz_{i,j}^y|x_i,a_{i,j}) p^y_{\theta}(y_{i,j}|y_{i,j-1}, x_i, a_{i,j}, \vz_{i,j}^y) \nonumber
\end{eqnarray}

Next, we describe how we operationalise the probability terms in Equation~\ref{eqn:probgen} using neural architectures, and how we learn the model parameters using the variational approach to overcome the challenges of integration over the latent variables. 

%The global planning decoder takes $\mathbf{z}^a$ as initial input, and at time step $t$, it decodes a dialogue act $a_t$. Then, the utterance generator produces corresponding sentence, considering both the input $x_t$, the dialogue act $a_t$, and local latent variable $\mathbf{z}^y$ (Figure~\ref{fig:framework}). The planning process decomposes the long dialogue synthetic process into a series of context-dependent sentence generation sub-tasks. 
% It could manage the generation process in a precise way, depending on the hierarchical variational latent structures. 

%At decoder side, ground truth $y$ is encoded in the similar way.

%The hidden representation of input data is formulated as $\mathbf{h}_{x} = \{\mathbf{h}_{{x}_{1}},...,\mathbf{h}_{{x}_{n}}\}$.
%For each representation of ${\bf h}_{x_i}$, it is embedded through BART model following with a Average pooling operation~\cite{cer2018universal}: $\mathbf{h}_{x_i} = \text{Avgpool}({\rm BART}(x_i))$. At decoder side, ground truth $y$ is encoded in the similar way.

% % Take pre-trained model as intial representation: aT-2/BART. (Details omitted temporarily for further development)

\subsection{Global Planning with Dialogue Acts}
\label{globalgeneration}
Dialogue acts describe the basic function of a dialogue utterance (\eg\ inform, clarification), and {reflect user intents~\cite{stolcke2000dialogue,bunt2011semantics}.} Synthetic dialogue generation task is not only about sentence generation, but also incorporating dialogue-specific features. Dialogue acts, as one of representatives in dialogue features,  play an important role in the generation of synthetic pseudo dialogues. In the \textit{FloDial} dataset, for each utterance $y_{i,j}$, there is a corresponding dialogue act tag.
%%which can be regarded as high-level sketch for detailed utterance generation.

We employ a global planning process to generate a sequence of dialogue acts.
% Prior to global planning, we use the pre-trained model BART~\cite{lewis2020bart} to initialize our representation of the input data $x = \{x_1, x_2,...,x_n\}$. The hidden representation of input data is formulated as
% $\mathbf{h}_{x} = \{\mathbf{h}_{{x}_{1}},...,\mathbf{h}_{{x}_{n}}\}$.
% \reza{do you mean $\mathbf{h}^x$ to be the 'collection' of $\mathbf{h}_i^x$? In the rest of this section, you have used $\mathbf{h}^x$ in the conditioning context of the probabilities, so not sure whether it should be a sequence of vectors or just a vector? Also, each $x_i$ is a 'sequence' of words (corresponding to the text in a node together with the user response on the outgoing edge), right? then when $x_i$ is fed to BERT, in fact a sequence is fed into BERT?}
%
%The global planning process can be formulated as follows:
%\begin{align*}
%    a_t = \text{argmax} P(a_t |a_{<t}, \mathbf{h}^{x}, \mathbf{z}^a)
%\end{align*}
%where $a = \{a_1,...a_n\}$ is a sequence of dialogue acts. 
%
Specifically, we inject stochasticity to this process using a continuous latent variable in each dialogue turn
%To construct the global planning latent variable 
$\vz^a_i$, which is assumed to follow the isotropic Gaussian distribution~\cite{kingma2014auto}. Given Gaussian  prior distributions 
$p_\theta^{\vz^a} (\vz^a_i | x_i)$, 
we propose to approximate the  posterior distribution $q_\phi (\vz^a_i  | x_i, y_i)$ using Gaussians in the  training phase.
% The global planning latent variable $\mathbf{z}^a$ is assumed to follow the Gaussian distribution~\cite{kingma2014auto}, and the prior and posterior distributions are formulated by $p_\theta (\mathbf{z}_a | \mathbf{h}^{x})$ and $q_\phi (\mathbf{z}_a | \mathbf{h}^{x}, \mathbf{h}^{y})$ respectively. 
The parameters $\bm{\mu}^{p}_{a}$, $\bm{\sigma}^{p}_{a}$,  $\bm{\mu}^{q}_{a}$ and $\bm{\sigma}^{q}_{a}$ of the prior and posterior distributions are parameterised with neural networks as follows:

\vspace{-5mm}
{
\begin{align*}
    & \bm{\mu}^p_{a} = \text{MLP}^p_\theta({\vh^{x}_i}),
    \bm{\sigma}^p_{a} = \text{softplus}(\text{MLP}^p_\theta(\vh^{x}_i)), \\
    & \bm{\mu}^q_{a} = \text{MLP}^q_\phi([{\vh^{x}_i,\vh^{y}_i]}),  \\
    &\bm{\sigma}^q_{a} = \text{softplus}(\text{MLP}^q_\phi([\vh^{x}_i,\vh^{y}_i])),
\end{align*}
}
%
\hspace*{-2mm}where ${\rm MLP}(\cdot)$ denotes a multi-layer perceptron, and ${\rm softplus(\cdot)}$ is a smooth approximation to ReLU, which ensures positiveness.
%
Each $x_i$ is fed into the encoder of the BART model ~\cite{lewis2020bart}, and followed by an average pooling operation~\cite{cer2018universal} to get its representation: $\vh_i^{x} = \text{AvgPool}({\rm BART}(x_i))$. 
%
We use a similar process to encode each utterance $y_{i,j}$ in the $i$-th turn, and then apply average pooling over the resultant representations in this turn to get $\vh_i^y$.

The Evidence Lower Bound (ELBO) is computed as follows:
%\footnote{See the derivation  in the Appendix.}, 
%\vspace*{-2mm}
\begin{eqnarray*}
  \lefteqn{\mathcal{L}_{\mathrm{global}}  =  -D_{KL}(q_\phi({\vz}^{a}_i|{x}_i, {y}_i)||p_\theta^{\vz^a}({\vz}^{a}_i|{x}_i))} \\
    & & + \mathbb{E}_{{\vz}^{a}_i \sim q_\phi}[\sum_j \log p_{\theta}^a({a_{i,j}} |a_{i,j-1},{\vz}^{ a}_i,{x}_i)]
   % \vspace*{-2mm}
\end{eqnarray*}
where $D_{KL}(\cdot |\cdot)$ refers to Kullback-Leibler divergence~\cite{kullback1951information}.
%
The dialogue act probability function $p_{\theta}^a(a_{i,j} |a_{i,j-1}, {\vz}^{ a}_i,\vh^{x}_i)$ is a 2-layer MLP with the softmax on top. 
%

%At time step $t$, A sample of ${\bf z}^{a}$ using the reparametrization
%trick~\cite{kingma2014auto} is then fed into the global planning decoder. Each $a_{t}$ is decoded by calculating the probability $P(a_{t} | a_{<t}, {\bf h}_{x_t}, {\bf z}^{a})$. The training loss function at time step $t$ is formulated as:
%\begin{eqnarray*}
%  \lefteqn{-\log P(a_{t}=\hat{a}_{t} | a_{<t}, \textbf{h}^{x},{\bf z}^{\bf a})} \\
%     &= & - \sum_{a_{t} = \hat{a}_{t}} \log P(a_{t}) 
%     - \sum_{a_{t} \neq \hat{a}_{t}} \log(1 - P(a_{t})).
%\end{eqnarray*}

\subsection{Local Planning for Utterance Generation}
\label{localgeneration}
The local sentence planning module aims to generate lexically diverse dialogue utterances $\vy = \{y_1,y_2,...,y_n\}$ that are faithful to the flowchart. For the $j$-th utterance in the $i$-th turn $y_{i,j}$, the utterance decoder considers the information corresponding to the node in the flowchart $x_i$, the corresponding dialogue act $a_{i,j}$ and the local planning variable $\vz^y_{i,j}$ by sampling the utterance from $p^y_{\theta}(.|y_{i,j-1}, x_i, a_{i,j}, \vz_{i,j}^y)$.
%\begin{align*}
%    y_t = \text{argmax} P (y_t | y_{<t}, \mathbf{h}^{x}, \mathbf{h}^{a}, \mathbf{z}^y),
%\end{align*}
%
We provide the representation of the conditioning context to the BART encoder, and generate the utterance via the decoder. 
%
We simply concatenate (non-linear transformation) the following: $\vh_{i,j-1}^y, \vz_{i,j}^y, \vh_i^x$ and $ \vh^a_{i,j}$, which is the embedding of the dialogue act $a_{i,j}$. The BART decoder then attends to these  vectors to generate the output utterance.  

The construction of local planning latent variable ${\vz}^{y}_{i,j}$ is similar to that of the global latent variable. We assume that it follows the Gaussian distribution.
%cal plannThe loing process is similar to the global planning process. The local planning latent variable $z^y$ is assumed to follow the Gaussian distribution $\mathcal{N}({\bf \mu},{\bf \sigma^{2}I})$. and 
The prior and posterior distributions are formulated by $
p_\theta^{\vz^y} (\vz^y_{i,j} | x_i, a_{i,j})$ and $q_\phi (\vz^y_{i,j} | x_i, a_{i,j}, y_{i,j})$, and they are parameterised as follows:
{
\begin{eqnarray*}
\bm{\mu}^p_{y} & = & \text{MLP}^p_\theta({\vh}^{x}_i,\vh^a_{i,j}), \\
\bm{\sigma}^p_{y} & = &\text{softplus}(\text{MLP}^p_\theta({\vh}^{x}_i,\vh^a_{i,j})\\
\bm{\mu}^q_{y} & = & \text{MLP}^q_\phi({\vh}^{x}_i,\vh^a_{i,j},\vh^y_{i,j}), \\ \bm{\sigma}^q_{y}
& = & \text{softplus}(\text{MLP}^q_\phi({\vh}^{x}_i,\vh^a_{i,j},\vh^y_{i,j}).
\end{eqnarray*}
}

%The decoder for utterance generation is also initialized by the BART model. For the $j$-th word in $y_t$ utterance, the word $y_t^{j}$ is decoded on the condition $\{y_t^{\textless j}, y_{<t}, \mathbf{h}^{x}, a, \mathbf{z}^y\}$. 
The ELBO for local planning is:
\vspace*{-2mm}\begin{eqnarray*}
    \lefteqn{\mathcal{L}_{\mathrm{local}} =}\\
    & & \!\!\!-D_{KL}(q_\phi({\vz}^{y}_{i,j}|{x}_i,a_{i,j}, y_{i,j})||p_\theta^{\vz^y}({\vz}^{y}_{i,j}|{x}_i,a_{i,j})) \\
    & & \!\!\!+\mathbb{E}_{{\vz}^{y}_{i,j} \sim q_\phi}[\log p_{\theta}({y}_{i,j} |y_{i,j-1}, x_i, a_{i,j}, \vz^y_{i,j})].
\end{eqnarray*}

The overall training objective to be optimised is the  sum of the ELBOs:
$\mathcal{L}_{\mathrm{all}} = \mathcal{L}_{\mathrm{global}} + \mathcal{L}_{\mathrm{local}}.$
We use the reparametrization
trick in~\cite{kingma2014auto} to optimise  the training objective. 













==> method_new_back.tex <==
\section{Pseudo Dialogue Synthesis}

\subsection{Task Formulation}
Given a sub-path ${x} = \{{x}_1, {x}_2, \ldots, {x}_n\}$ in a flowchart as input, where each $x_i$ is a question-answer pair in the flowchart (e.g., ``starter cranks? No'' in Figure~\ref{fig:intro}) or a problem statement, our task is to generate a long and diverse synthetic pseudo conversation ${y} = \{{y}_1, {y}_2, \ldots, {y}_n\}$ where ${y}_i$ is the $i$-th turn in this dialogue, and a sequence of corresponding dialogue acts ${a} = \{{a}_1, {a}_2, \ldots, {a}_n\}$.
% \reza{what's the relation between $n$ and $m$? why the dialogue acts 'a' are boldface here, but not in the rest of the section? why 'x' is bold here but not bold in the rest of the section?}
% \haolan{To avoid misunderstanding, I just keep the same number of x, y, a. In our implementation, the input is actually ($x_1, x_2, x_2, x_3, x_3, ....$)}

% Given input data $x = \{x_1, x_2,...,x_n\}$ where each $x_i$ can be an short prompt sentence or instruction (e.g., flowchart node description), our task is to generate a long and diverse pseudo dialogue content $y = \{y_1,y_2,...,y_m\}$ that $y_i$ is the $i$-th utterance of generative pseudo dialogue, and a sequence of dialogue act (DA) $a = \{a_1, a_2,...,a_m\}$. The generative pseudo dialogue content should follow the plan and order of input prompt sentence. For each of the $y_i$ and its corresponding dialogue act $a_i$, it might contains 1 to 3 sub-sentences and sub-dialogue acts, e.g. $y_i = <y_i^1,...,y_i^j>$ and $a_i = <a_i^1,...,a_i^j>$, while $j \in [1,3]$.

% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.95\linewidth]{images/overall.pdf}
% \label{screenshot}
% \vspace{-3mm}
% \caption{Overall graphical model of our proposed model.}
% \label{fig:overall}
% \end{figure}

\begin{figure*}
\centering
\includegraphics[width=0.9\linewidth]{images/new_framework.jpg}
\label{screenshot}
\vspace{-3mm}
\caption{Detailed architecture of the VarDA model.}
\label{fig:framework}
\end{figure*}

\subsection{Approach Overview}
Our approach devises a variational data augmentation model (VarDA) with hierarchical planning strategy. It contains two planning latent variables: global planning latent variable $\mathbf{z}^a$ and local planning latent variable $\mathbf{z}^y$. The global planning latent variable $\mathbf{z}^a$ is responsible for modeling the dialogue act transition process (e.g., inform, Yes-No-question, clarify), also known as high-level sketch. The local planning latent variable $\mathbf{z}_y$ is responsible for generating lexically diverse utterances to realize dialogue acts, also known as low-level realization.

The global planning decoder takes $\mathbf{z}^a$ as initial input, and at time step $t$, it decodes a dialogue act $a_t$. Then, the utterance generator produces corresponding sentence, considering both the input $x_t$, the dialogue act $a_t$, and local latent variable $\mathbf{z}^y$ (Figure~\ref{fig:framework}). The planning process decomposes the long dialogue synthetic process into a series of context-dependent sentence generation sub-tasks. 
% It could manage the generation process in a precise way, depending on the hierarchical variational latent structures. 

\subsection{Input Representation}
We use the pre-trained model BART~\cite{lewis2020bart} to initialize our representation for input data $x = \{x_1, x_2,...,x_n\}$ where each $x_i$ contains a sequence of words.  The hidden representation of input data is formulated as $\mathbf{h}_{x} = \{\mathbf{h}_{{x}_{1}},...,\mathbf{h}_{{x}_{n}}\}$.
For each representation of ${\bf h}_{x_i}$, it is embedded through BART model following with a Average pooling operation~\cite{cer2018universal}: $\mathbf{h}_{x_i} = \text{Avgpool}({\rm BART}(x_i))$. At decoder side, ground truth $y$ is encoded in the similar way.

% % Take pre-trained model as intial representation: aT-2/BART. (Details omitted temporarily for further development)

\subsection{Global Planning with Dialogue Act}
Dialogue acts describe the function of dialogue utterance, and reflect a user's intent. Therefore, dialogue acts play an important role in the generation of synthetic pseudo dialogues. %%which can be regarded as high-level sketch for detailed utterance generation.
As mentioned above, we employ a global planning process to generate a sequence of dialogue acts.
% Prior to global planning, we use the pre-trained model BART~\cite{lewis2020bart} to initialize our representation of the input data $x = \{x_1, x_2,...,x_n\}$. The hidden representation of input data is formulated as
% $\mathbf{h}_{x} = \{\mathbf{h}_{{x}_{1}},...,\mathbf{h}_{{x}_{n}}\}$.
% \reza{do you mean $\mathbf{h}^x$ to be the 'collection' of $\mathbf{h}_i^x$? In the rest of this section, you have used $\mathbf{h}^x$ in the conditioning context of the probabilities, so not sure whether it should be a sequence of vectors or just a vector? Also, each $x_i$ is a 'sequence' of words (corresponding to the text in a node together with the user response on the outgoing edge), right? then when $x_i$ is fed to BERT, in fact a sequence is fed into BERT?}
The global planning process can be formulated as follows:
\begin{align*}
    a_t = \text{argmax} P(a_t |a_{<t}, \mathbf{h}^{x}, \mathbf{z}^a)
\end{align*}
where $a = \{a_1,...a_n\}$ is a sequence of dialogue acts. To construct the global planning latent variable $\mathbf{z}^a$ which is assumed to follow the isotropic Gaussian distribution~\cite{kingma2014auto}, we propose to approximate the true (prior) distribution $p_\theta (\mathbf{z}_a | \mathbf{h}^{x})$ with a posterior distribution $q_\phi (\mathbf{z}_a | \mathbf{h}^{x}, \mathbf{h}^{y})$ in the  training phase.
% The global planning latent variable $\mathbf{z}^a$ is assumed to follow the Gaussian distribution~\cite{kingma2014auto}, and the prior and posterior distributions are formulated by $p_\theta (\mathbf{z}_a | \mathbf{h}^{x})$ and $q_\phi (\mathbf{z}_a | \mathbf{h}^{x}, \mathbf{h}^{y})$ respectively. 
where the parameters $\bm{\mu}^{p}$, $\bm{\sigma}^{p}$,  $\bm{\mu}^{q}$ and $\bm{\sigma}^{q}$ of prior and posterior distributions are estimated by:
\begin{align*}
    & \bm{\mu}^p_{a} = \text{MLP}^p_\theta({\mathbf{h}^{x}}),  \bm{\sigma}^p_{a} = \text{softplus}(\text{MLP}^p_\theta(\mathbf{h}^{x})), \\
    & \bm{\mu}^q_{a} = \text{MLP}^q_\phi([{\mathbf{h}^{x},\mathbf{h}^{y}]}),  \bm{\sigma}^q_{a} = \text{softplus}(\text{MLP}^q_\phi([\mathbf{h}^{x}, \mathbf{h}^{y}])),
\end{align*}
where ${\rm MLP}(\cdot)$ denotes multiple layer perception, and ${\rm softplus(\cdot)}$ is a smooth approximation to ReLU, which ensures positiveness.
We give the Evidence Lower Bound (ELBO) as follows, which derivation can be found in the Appendix:
\begin{eqnarray*}
    \mathcal{L}_{\mathrm{global}} & = & -D_{KL}(q_\phi({\bf z}^{\bf a}|{\bf h}^{x}, {\bf h}^{y})||p_\theta({\bf z}^{\bf a}|{\bf h}^{x})) \\
    & & + \mathbb{E}_{{\bf z}^{\bf a} \sim q_\phi}[\log p_{\theta}({a} |{\bf z}^{\bf a},\textbf{h}^{x})]
\end{eqnarray*}
where $D_{KL}(\cdot |\cdot)$ refers to Kullback-Leibler divergence~\cite{kullback1951information}.

At time step $t$, A sample of ${\bf z}^{a}$ using the reparametrization
trick~\cite{kingma2014auto} is then fed into the global planning decoder. Each $a_{t}$ is decoded by calculating the probability $P(a_{t} | a_{<t}, {\bf h}_{x_t}, {\bf z}^{a})$. The training loss function at time step $t$ is formulated as:
\begin{eqnarray*}
  \lefteqn{-\log P(a_{t}=\hat{a}_{t} | a_{<t}, \textbf{h}^{x},{\bf z}^{\bf a})} \\
     &= & - \sum_{a_{t} = \hat{a}_{t}} \log P(a_{t}) 
     - \sum_{a_{t} \neq \hat{a}_{t}} \log(1 - P(a_{t})).
\end{eqnarray*}

\subsection{Local Planning for Utterance Generation}
The local sentence planning module aims to generate lexically diverse dialogue utterances $y = \{y_1,y_2,...,y_n\}$ that are faithful to the flowchart. For each utterance $y_t$, the utterance decoder considers the information corresponding to a node in the flowchart $x_i$, the corresponding dialogue act $a_i$ and the local planning variable $z^y$ by computing:
\begin{align*}
    y_t = \text{argmax} P (y_t | y_{<t}, \mathbf{h}^{x}, \mathbf{h}^{a}, \mathbf{z}^y),
\end{align*}
where  $\mathbf{h}^{a}$ is the hidden representation of dialogue act through encoder (as shown in Figure~\ref{fig:framework}). Construction of local planning latent variable ${\bf z}^{y}$ is similar to the previous global planning variable. It's also assumed to follow the Gaussian distribution.
%cal plannThe loing process is similar to the global planning process. The local planning latent variable $z^y$ is assumed to follow the Gaussian distribution $\mathcal{N}({\bf \mu},{\bf \sigma^{2}I})$. and 
The prior and posterior distributions are formulated by $p_\theta (\textbf{z}^y | y_{<t}, \textbf{h}_x, \textbf{h}_a)$ and $q_\phi (\textbf{z}^y |y_{<=t}, \textbf{h}_x, \textbf{h}_a)$. The parameters in prior  distribution are estimated by:
$\bm{\mu}^p_{y} = \text{MLP}^p_\theta({\bf h}^{x},\textbf{h}_a,{\bf h}^{y}_{<t}),  \bm{\sigma}^p_{y} = \text{softplus}(\text{MLP}^p_\theta({\bf h}^{x},\textbf{h}_a,{\bf h}^{y}_{<t})),$ while the posterior distribution: $\bm{\mu}^q_{y} = \text{MLP}^q_\phi({\bf h}^{x},\textbf{h}_a,{\bf h}^{y}_{\leq t}),  \bm{\sigma}^q_{y} = \text{softplus}(\text{MLP}^q_\phi({\bf h}^{x},\textbf{h}_a,{\bf h}^{y}_{\leq t}).$

The decoder for utterance generation is also initialized by the BART model. \reza{how does the decoder exactly works by conditioning?} It decodes a specific utterance $y_i$ conditioned on $\{ y_{<t}, \mathbf{h}^{x}, a, \mathbf{z}^y\}$. We give the ELBO for local planning as follows:
\begin{eqnarray*}
    \lefteqn{\mathcal{L}_{\mathrm{local}} =}\\
    & & -D_{KL}(q_\phi({\bf z}^{\bf y}|{\bf h}^{x},{ a},{\bf h}^{y}_{<t})||p_\theta({\bf z}^{\bf y}|{\bf h}^{x},{ a},{\bf h}^{y}_{\leq t})) \\
    & & +\mathbb{E}_{{\bf z}^{\bf y} \sim q_\phi}[\log p_{\theta}({y}_{t} |y_{<t}, \mathbf{h}^{x}, a, \mathbf{z}^y)].
\end{eqnarray*}

The overall training objective to be maximized is the  sum of the ELBOs:
$\mathcal{L}_{\mathrm{all}} = \mathcal{L}_{\mathrm{global}} + \mathcal{L}_{\mathrm{local}}.$


\subsection{Inference}
At inference stage, VarDA model will generate the dialogue context step by step. Specifically, at time step $t$, VarDA takes $x_t$ as input, then it generates a corresponding dialogue act $a_t$ by considering the input representation $\textbf{h}_{x_t}$ and sampled global latent variable $\textbf{z}^{a}$. Then, it generates its corresponding dialogue utterance $y_t$ by considering the input representation $\textbf{h}_{x_t}$, the representation of dialogue act $\textbf{h}_{a_t}$, local latent variable $\textbf{z}^{y}$ and previous generated utterance $y_{<t}$. VarDA will finish generation process when there is no more input information. The inference process is as follows:

(1) Sample global latent variable: $\textbf{z}^{a} \sim p_{\theta}(\textbf{z}^{a} | \textbf{h}_{x_t})$
\reza{should it be $\textbf{z}^{a_t}$ instead of $\textbf{z}^{a}$ ?}

(2) Predict corresponding dialogue act: $a_t \sim p_{\theta}(a_{t} | a_{<t}, \textbf{h}^{x},{\bf z}^{\bf a})$
\reza{should it be $\textbf{h}^{x_t}$ instead of $\textbf{h}^{x}$ ?}

(3) Sample local latent variable:  $\textbf{z}^{y} \sim p_{\theta}(\textbf{z}^{y} | \textbf{h}_{x_t}, \textbf{h}_{a_t})$
\reza{should it be $\textbf{z}^{y_t}$ instead of $\textbf{z}^{y}$ ?}

(4) Generate utterance: $y_t \sim p_{\theta}({y}_{t} |y_{<t}, \mathbf{h}^{x}, a, \mathbf{z}^y)$.
\reza{should it be $p_{\theta}({y}_{t} |y_{<t}, \mathbf{h}^{x_t}, a_t, \mathbf{z}^{y_t})$ ?}













==> method_yufei.tex <==
\section{Planning-based Data Augmentation}
In this section, we first introduce the task formulation in \S~\ref{formulation}. We then describe flowchart path extraction in \S~\ref{pathextract}. We further describe the overall of \da in \S~\ref{overviewda} as well as its planning module and training objective in \S~\ref{planning} and \S~\ref{trainingobj}, respectively. Figure~\ref{fig:framework} shows the overview of \da.

\subsection{Task Formulation}
\label{formulation}
The goal of \da is to take a sampled path from the flowchart, and generate a complete synthetic dialogue as well as the dialogue acts. In this paper, we only have access to a handful training set $\gT=\{(\vx,\va,\vy)_i\}_{i=1}^m$ where ${\vx} = \{{x}_1, {x}_2, \ldots, {x}_n\}$ is a flowchart \reza{sub-path}\noteRH{sub-path or path?}. Each flowchart node $x_i$ in this \reza{sub-path}\noteRH{sub-path or path?} corresponds to a sub-dialogue $y_i=[y_{i, 0}, \cdots, y_{i, |y_i|}] \in \vy$ where $y_{i,j}$ is an utterance with a dialogue act $a_{i,j} \in \va$. \reza{For example, the node ``battery over 12V'' in the flowchart path in Figure \ref{fig:intro} corresponds to the sub-dialogue starting from the 4th turn and ending in the 7th turn (highlighted by ``blue''). }


Given a flowchart \reza{sub-path}\noteRH{sub-path or path?} $\vx$, our proposed \emph{Data Augmentation} method \da generates synthetic dialogue acts $\hat{\va}$ and dialogues $\hat{\vy}$ and produces the final synthetic dataset $\gT_{Syn}=\{(\vx, \hat{\va},\hat{\vy})_i\}_{i=1}^n$ where $n$ could be much larger than $m$ (e.g., 10x). Our goal is that the downstream retrieval and generative dialogue models trained using $\gT \cup \gT_{Syn}$ outperform the ones only trained using $\gT$. 


% each $x_i$ is a question-answer pair in the flowchart (\eg\ ``starter cranks? No'' in Figure~\ref{fig:intro}) or a problem statement phrase (\eg\ car won't start)


% {We are given} a sub-path  in a flowchart as input, where  .
% %
% Our task is to generate a diverse synthetic pseudo conversation ${\vy} = \{{y}_1, {y}_2, \ldots, {y}_n\}$ where ${y}_i$ is the $i$-th turn in this dialogue.
% %
% We assume that  $y_i$ in the $i$-th turn consists of several utterances $\{y_{i,j}\}_{j=1}^{|y_i|}$ where each utterance has its own dialogue act $a_{i,j}$. As such, {we can capture} the multiple dialogue acts setting in a single turn. We denote the sequence of {dialogue acts by} $\va = \{a_1,..,a_n\}$ where $a_i = \{a_{i,j}\}_{j=1}^{|a_i|}$, {and $a_{i,j}$ is the dialogue act of corresponding utterance $y_{i,j}$.}  


\begin{figure*}
\centering
\includegraphics[width=1\linewidth]{images/acl2023_method_new.pdf}
\label{screenshot}
\vspace{-3mm}
\caption{Detailed architecture of the PlanDA model.}
\label{fig:framework}
\end{figure*}

\subsection{Flowchart Path Extraction}
\label{pathextract}
As shown in Figure~\ref{fig:intro}, the flowcharts used in this paper consist of decision nodes and action nodes. The decision nodes include question and they are connected with others by the user responses (e.g., Yes, No). The action nodes are at the bottom of the flowcharts indicating appropriate actions. For training, we directly extract the flowchart paths in the training data. For syntactic data generation, to ensure the full coverage for the flowchart paths, we extract the flowchart paths by the \emph{Depth-First-Search} from the top decision nodes until and bottom action nodes. The resulting flowchart paths are then used as the inputs for \da.




\subsection{Overview of \da}
\label{overviewda}
Given the extracted flowchart paths, \da is designed to generate diverse and high-quality synthetic dialogues. Although the input flowchart paths include textual questions, user responses and final actions,  conditioning only on these information could result in tedious conversations (\eg\  consisting only of a series of question-answer pairs). In fact, given a node in the flowchart, there could be many feasible open-ended dialogues. To cover the feasible dialogue space, one could use intermediate variables in \da. In the context of dialogue, \emph{dialogue acts}  describe the basic function of a dialogue turn/utterance (\eg\ inform, clarification), and reflect user intents~\cite{stolcke2000dialogue,bunt2011semantics}. 
%
\reza{In our model,  dialogue acts  intuitively characterise the intermediate (latent) variables discussed above.}
%They should be perfect candidates for characterising the intermediate variables discussed above. Thus, we propose to use dialogue acts as  planning variables in \da.

\reza{\da is a Seq2Seq-based model that, 
%is equiped with the internal dialogue act planning module.
generates the sub-dialogue $y_i$, in a auto-regressive manner, for a given flowchart node $x_i$. It conditions on $x_i$ and previously generated utterances $y_{i,j-1}$ to generate diverse and high-quality synthetic utterances $y_{i,j}$.} Specifically, \da first encodes $x_i$ and $y_{i,j-1}$, then its planning module produces a sequence of planning vectors $[\vh^z_{i,0}, \cdots, \vh^z_{i,|y_i|}]$ conditioned on $x_i$. Finally, \da generates each utterance $y_{i,j}$ based on $\vh^z_{i,j}$, $x_i$ and $y_{i,j-1}$, as follows:
\begin{align}
    \vh^x_i &= \mathit{AvgPool}(\mathit{Enc}(x_i)) \\
    \vh^y_{i,j-1} &= \mathit{AvgPool}(\mathit{Enc}(y_{i,j-1})) \\
    [\vh^z_{i, 0}, \cdots, \vh^z_{i,|y_i|}] &= \mathit{Plan}(\vh^x_i) \label{plan} \\ 
    y_{i,j} &= \mathit{Dec}(\vh^y_{i,j-1}, \vh^x_i, \vh^z_{i,j})
\end{align}
where $\mathit{Enc}$ and $\mathit{Dec}$ are based on the Transformer architecture and their parameters are initialized from the pre-trained Seq2Seq model (e.g., BART). 

\subsection{Planning Module in \da}
\label{planning}
Next, we describe the internal planning design in Equation~\ref{plan}. \da has a hierarchical planning strategy with 
global planning latent variable $\mathbf{z}^a_i$ and local planning latent variable $\mathbf{z}^y_{i,j}$. $\mathbf{z}^a_i$ is responsible for modeling the {dialogue act transition process \emph{{over the turns}}}, while $\mathbf{z}^y_{i,j}$ is responsible for generating lexically diverse utterances. 

\paragraph{Global Planning over Dialogue Acts}
In the global planning, we inject stochasticity to this process using a continuous latent variable in each dialogue turn
$\vz^a_i$, which is assumed to follow the isotropic Gaussian distribution~\cite{kingma2014auto}. We first sample $\mathbf{z}^a_i$ from its prior distribution $p_\theta^{\vz^a} (\vz^a_i | x_i)$ and then generate a sequence of dialogue acts auto-repressively:
\begin{align}
    \vz^a_i&~\sim~p_\theta^{\vz^a} (\vz^a_i | x_i) \\
    a_{i,j}&=p^{a}_{\theta}(. | a_{i,j-1}, x_i,\vz^a_i)
\end{align}
where $p_{\theta}^a(a_{i,j} |a_{i,j-1}, {\vz}^{ a}_i,\vh^{x}_i)$ is a 2-layer MLP with the softmax on top. We train $p_\theta^{\vz^a} (\vz^a_i | x_i)$ to approximate the  posterior distribution $q_\phi (\vz^a_i  | x_i, y_i)$ using Gaussians in the training phase. The parameters in prior and posterior distributions, $\bm{\mu}^{p}_{a}$, $\bm{\sigma}^{p}_{a}$,  $\bm{\mu}^{q}_{a}$ and $\bm{\sigma}^{q}_{a}$, are parameterised as follows:
\begin{align}
    \bm{\mu}^p_{a} &= \mathit{MLP}^p_\theta({\vh^{x}_i}), \\
    \bm{\sigma}^p_{a} &= \mathit{softplus}(\mathit{MLP}^p_\theta(\vh^{x}_i)), \\
    \bm{\mu}^q_{a} &= \mathit{MLP}^q_\phi([{\vh^{x}_i,\vh^{y}_i]}), \\
    \bm{\sigma}^q_{a} &= \mathit{softplus}(\mathit{MLP}^q_\phi([\vh^{x}_i,\vh^{y}_i])), 
\end{align}
where ${\rm MLP}(\cdot)$ denotes a multi-layer perceptron, ${\rm softplus(\cdot)}$ is a smooth approximation to ReLU, which ensures positiveness and $\vh^{y}_i=\mathit{AvgPool}(\mathit{Enc}([y_{i, 0}, \cdots, y_{i, k}]))$ allowing $\vz^a_i$ to capture the global utterance information associated with $x_i$. Finally, the Evidence Lower Bound (ELBO) is computed as follows:
\begin{eqnarray*}
  \lefteqn{\mathcal{L}_{\mathrm{global}}  =  -D_{KL}(q_\phi({\vz}^{a}_i|{x}_i, {y}_i)||p_\theta^{\vz^a}({\vz}^{a}_i|{x}_i))} \\
    & & + \mathbb{E}_{{\vz}^{a}_i \sim q_\phi}[\sum_j \log p_{\theta}^a({a_{i,j}} |a_{i,j-1},{\vz}^{ a}_i,{x}_i)]
\end{eqnarray*}
where $D_{KL}(\cdot |\cdot)$ refers to Kullback-Leibler divergence~\cite{kullback1951information}.

% The generation process works as follows:
% \begin{itemize}
% \itemsep0em
%     \item Sample the  dialogue act:\\  $a_{i,j}~\sim~p^{a}_{\theta}(. | a_{i,j-1}, x_i,\vz^a_i)$
%     \item Sample the local latent variable:\\
% $\vz^{y}_{i,j}~\sim~p^{\vz^y}_{\theta}(. | x_i, a_{i,j})$   
% \item Sample the utterance:\\
%  $y_{i,j}~\sim~p^y_{\theta}(.|y_{i,j-1}, x_i, a_{i,j}, \vz_{i,j}^y)$
% \end{itemize}
% As the $\vz$ variables are continuous latent variables, the probability of generating a conversation and the corresponding dialogue acts given the flowchart path can be written as follows:
% \begin{eqnarray}
% \label{eqn:probgen}
% \lefteqn{p_{\theta}(\vy,\va|\vx) = \prod_i  \int d(\vz_i^a)  p_{\theta}^{\vz^a}(\vz_i^a|x_i)}  \\  
%     &&  \times \prod_j \int d(\vz_{i,j}^y)    p_{\theta}^a(a_{i,j}|a_{i,j-1},x_i, \vz_i^a) \nonumber \\ 
%     && \times p_{\theta}^{\vz^y}(\vz_{i,j}^y|x_i,a_{i,j}) p^y_{\theta}(y_{i,j}|y_{i,j-1}, x_i, a_{i,j}, \vz_{i,j}^y) \nonumber
% \end{eqnarray}

%  Given Gaussian  prior distributions 
% $p_\theta^{\vz^a} (\vz^a_i | x_i)$, 
% we propose to approximate the  posterior distribution $q_\phi (\vz^a_i  | x_i, y_i)$ using Gaussians in the  training phase.
% % The global planning latent variable $\mathbf{z}^a$ is assumed to follow the Gaussian distribution~\cite{kingma2014auto}, and the prior and posterior distributions are formulated by $p_\theta (\mathbf{z}_a | \mathbf{h}^{x})$ and $q_\phi (\mathbf{z}_a | \mathbf{h}^{x}, \mathbf{h}^{y})$ respectively. 
% The parameters $\bm{\mu}^{p}_{a}$, $\bm{\sigma}^{p}_{a}$,  $\bm{\mu}^{q}_{a}$ and $\bm{\sigma}^{q}_{a}$ of the prior and posterior distributions are parameterised with neural networks as follows:
% \begin{align*}

%     \bm{\mu}^p_{a} &= \text{MLP}^p_\theta({\vh^{x}_i}), \\
%     \bm{\sigma}^p_{a} &= \text{softplus}(\text{MLP}^p_\theta(\vh^{x}_i)), \\
%     \bm{\mu}^q_{a} &= \text{MLP}^q_\phi([{\vh^{x}_i,\vh^{y}_i]}), \\
%     \bm{\sigma}^q_{a} &= \text{softplus}(\text{MLP}^q_\phi([\vh^{x}_i,\vh^{y}_i])), \\
% \end{align*}
% where ${\rm MLP}(\cdot)$ denotes a multi-layer perceptron, and ${\rm softplus(\cdot)}$ is a smooth approximation to ReLU, which ensures positiveness. 
%

% Each $x_i$ is fed into the encoder of the BART model ~\cite{lewis2020bart}, and followed by an average pooling operation~\cite{cer2018universal} to get its representation: $\vh_i^{x} = \text{AvgPool}({\rm BART}(x_i))$. 
% %
% We use a similar process to encode each utterance $y_{i,j}$ in the $i$-th turn, and then apply average pooling over the resultant representations in this turn to get $\vh_i^y$. 
% %
% The dialogue act probability function $p_{\theta}^a(a_{i,j} |a_{i,j-1}, {\vz}^{ a}_i,\vh^{x}_i)$ is a 2-layer MLP with the softmax on top. 



\paragraph{Local Planning for Utterance Generation}
Given the dialogue act $a_{i,j}$ generated from $\vz^a_i$, we then focus on generating lexically diverse dialogue utterances that are faithful to the flowchart. We sample $\mathbf{z}^y_{i,j}$ from its prior distribution conditioned on $a_{i,j}$ and $x_i$, as follows:
\begin{align}
    \vz^{y}_{i,j}~\sim~p^{\vz^y}_{\theta}(\vz^{y}_{i,j}| x_i, a_{i,j})
\end{align}
We train $p^{\vz^y}_{\theta}(\vz^{y}_{i,j}| x_i, a_{i,j})$  to approximate the  posterior distribution $q_\phi (\vz^y_{i,j} | x_i, a_{i,j}, y_{i,j})$. We assume that both distributions are Gaussians. They are parameterised as follows:
\begin{align}
\bm{\mu}^p_{y} &= \text{MLP}^p_\theta({\vh}^{x}_i,\vh^a_{i,j}), \\
\bm{\sigma}^p_{y} &= \text{softplus}(\text{MLP}^p_\theta({\vh}^{x}_i,\vh^a_{i,j})\\
\bm{\mu}^q_{y} &= \text{MLP}^q_\phi({\vh}^{x}_i,\vh^a_{i,j},\vh^y_{i,j}), \\ \bm{\sigma}^q_{y}
&= \text{softplus}(\text{MLP}^q_\phi({\vh}^{x}_i,\vh^a_{i,j},\vh^y_{i,j})).
\end{align}
where $h^a_{i,j}=\mathit{AvgPool}(\mathit{Enc}(a_{i,j}))$. Different from global planning, we use the ground-truth utterance $y_{i,j}$ for training to allow \da to focus on the local information. Finally, the ELBO for local planning variable is:
\vspace*{-2mm}\begin{eqnarray*}
    \lefteqn{\mathcal{L}_{\mathrm{local}} =}\\
    & & \!\!\!-D_{KL}(q_\phi({\vz}^{y}_{i,j}|{x}_i,a_{i,j}, y_{i,j})||p_\theta^{\vz^y}({\vz}^{y}_{i,j}|{x}_i,a_{i,j})) \\
    & & \!\!\!+\mathbb{E}_{{\vz}^{y}_{i,j} \sim q_\phi}[\log p_{\theta}({y}_{i,j} |y_{i,j-1}, x_i, a_{i,j}, \vz^y_{i,j})].
\end{eqnarray*}

\paragraph{Outputs of Planning Module}
The planning module in \da concatenates the results from global and local planning as the final outputs. The $\vh^z_{i,k}$ in Equation~\ref{plan} is defined as follows:
\begin{align}
    \vh^z_{i,k}=\text{Concat}([\vh^a_{i,j}, \vz^{y}_{i,j}])
\end{align}

\subsection{Training Objective}
\label{trainingobj}
Finally, in \da, the probability of generating a conversation and the corresponding dialogue acts given the flowchart path can be written as follows:
\begin{eqnarray}
\label{eqn:probgen}
\lefteqn{p_{\theta}(\vy,\va|\vx) = \prod_i  \int d(\vz_i^a)  p_{\theta}^{\vz^a}(\vz_i^a|x_i)}  \\  
    &&  \times \prod_j \int d(\vz_{i,j}^y)    p_{\theta}^a(a_{i,j}|a_{i,j-1},x_i, \vz_i^a) \nonumber \\ 
    && \times p_{\theta}^{\vz^y}(\vz_{i,j}^y|x_i,a_{i,j}) p^y_{\theta}(y_{i,j}|y_{i,j-1}, x_i, a_{i,j}, \vz_{i,j}^y) \nonumber
\end{eqnarray} 
The overall training objective of \da is the  sum of the ELBOs:
$\mathcal{L} = \mathcal{L}_{\mathrm{global}} + \mathcal{L}_{\mathrm{local}}.$
We use the reparametrization
trick in~\cite{kingma2014auto} to optimise the training objective.

% The local sentence planning module aims to generate lexically diverse dialogue utterances $\vy = \{y_1,y_2,...,y_n\}$ that are faithful to the flowchart. For the $j$-th utterance in the $i$-th turn $y_{i,j}$, the utterance decoder considers the information corresponding to the node in the flowchart $x_i$, the corresponding dialogue act $a_{i,j}$ and the local planning variable $\vz^y_{i,j}$ by sampling the utterance from $p^y_{\theta}(.|y_{i,j-1}, x_i, a_{i,j}, \vz_{i,j}^y)$.
% %\begin{align*}
% %    y_t = \text{argmax} P (y_t | y_{<t}, \mathbf{h}^{x}, \mathbf{h}^{a}, \mathbf{z}^y),
% %\end{align*}
% %
% We provide the representation of the conditioning context to the BART encoder, and generate the utterance via the decoder. 
% %
% We simply concatenate (non-linear transformation) the following: $\vh_{i,j-1}^y, \vz_{i,j}^y, \vh_i^x$ and $ \vh^a_{i,j}$, which is the embedding of the dialogue act $a_{i,j}$. The BART decoder then attends to these  vectors to generate the output utterance.  

% The construction of local planning latent variable ${\vz}^{y}_{i,j}$ is similar to that of the global latent variable. We assume that it follows the Gaussian distribution.
% %cal plannThe loing process is similar to the global planning process. The local planning latent variable $z^y$ is assumed to follow the Gaussian distribution $\mathcal{N}({\bf \mu},{\bf \sigma^{2}I})$. and 
% The prior and posterior distributions are formulated by $
% p_\theta^{\vz^y} (\vz^y_{i,j} | x_i, a_{i,j})$ and $q_\phi (\vz^y_{i,j} | x_i, a_{i,j}, y_{i,j})$, and they are parameterised as follows:

% \begin{eqnarray*}
% \bm{\mu}^p_{y} & = & \text{MLP}^p_\theta({\vh}^{x}_i,\vh^a_{i,j}), \\
% \bm{\sigma}^p_{y} & = &\text{softplus}(\text{MLP}^p_\theta({\vh}^{x}_i,\vh^a_{i,j})\\
% \bm{\mu}^q_{y} & = & \text{MLP}^q_\phi({\vh}^{x}_i,\vh^a_{i,j},\vh^y_{i,j}), \\ \bm{\sigma}^q_{y}
% & = & \text{softplus}(\text{MLP}^q_\phi({\vh}^{x}_i,\vh^a_{i,j},\vh^y_{i,j}).
% \end{eqnarray*}


% %The decoder for utterance generation is also initialized by the BART model. For the $j$-th word in $y_t$ utterance, the word $y_t^{j}$ is decoded on the condition $\{y_t^{\textless j}, y_{<t}, \mathbf{h}^{x}, a, \mathbf{z}^y\}$. 
% The ELBO for local planning is:
% \vspace*{-2mm}\begin{eqnarray*}
%     \lefteqn{\mathcal{L}_{\mathrm{local}} =}\\
%     & & \!\!\!-D_{KL}(q_\phi({\vz}^{y}_{i,j}|{x}_i,a_{i,j}, y_{i,j})||p_\theta^{\vz^y}({\vz}^{y}_{i,j}|{x}_i,a_{i,j})) \\
%     & & \!\!\!+\mathbb{E}_{{\vz}^{y}_{i,j} \sim q_\phi}[\log p_{\theta}({y}_{i,j} |y_{i,j-1}, x_i, a_{i,j}, \vz^y_{i,j})].
% \end{eqnarray*}



